Traffic Queue Length and Pressure Estimation for Road Networks with Geometric Deep Learning Algorithms

Due to urbanization and the increase of individual mobility, in most metropolitan areas around the world congestion and inefficient traffic management occur. Highly necessary intelligent traffic control systems, which are able to reduce congestion, rely on measurements of traffic situations in urban road networks and freeways. Unfortunately, the instrumentation for accurate traffic measurement is expensive and not widely implemented. This thesis addresses this problem, where relatively inexpensive and easy to install loop-detectors are used by a geometric deep learning algorithm, which uses loop-detector data in a spatial context of a road network, to estimate queue length in front of signalized intersections, which can be then used for following traffic control tasks. Therefore, in the first part of this work a conventional estimation method for queue length (which does not use machine learning techniques) based on second-by-second loop-detector data is implemented, which uses detected shockwaves in queues to estimate the length and point of time for the maximum queue. The method is later used as reference but also as additional input information for the geometric deep learning approach. In the second part the geometric deep learning algorithm is developed, which uses spatial correlations in the road network but also temporal correlations in detector data time sequences by new attention mechanisms, to overcome the limitations of conventional methods like excess traffic demand, lane changing and stop-and-go traffic. Therefore, it is necessary to abstract the topology of the road network in a graph. Both approaches are compared regarding their performance, reliability as well as limitations and validated by usage of the traffic simulation software SUMO (Simulation of Urban MObility). Finally, the results are discussed in the conclusions and further investigations are suggested.

==> 2stateofart/deeplearning.tex <==
\chapter{Queue Length Estimation with Geometric Deep Learning} \label{sec.geometric_deep_learning}

As demonstrated in section \ref{sec.liu_on_grid}, the estimation of the expansion model is not accurate for a realistic road network due to lane changes and stop and go traffic behavior. Therefore, in this work another approach with geometric deep learning will be examined. This approach is potential superior, since it is able to take spatial correlations into consideration due to graph attention mechanisms. Furthermore, it is expected the network is able to learn more complex relations like lane changing.
In the past few years a big progress was made in the field of \textit{neural sequence-to-sequence models}, especially applied to human language translation \cite{neubig_neural_2017}. The goal of this work is to apply these techniques on road networks for estimation and prediction of queue length and pressure. Generally, the model gets a time sequence containing of detector data as input and gives a time sequence of traffic queue length as output. 

In this chapter, the fundamentals which are important to implement geometric deep learning networks are presented. Furthermore, the implementation of the  deep learning network as well as the results are shown.

\section{Fundamentals of Geometric Deep Learning}

Deep learning approaches became very popular during the past decades, since they were successfully applied in many different fields to solve real-world problems. Especially deep learning had big achievements in the past in fields like human language translation, computer vision, robotics, search engines and many more. Deep learning is a name for a particular class of machine learning techniques. Many of the recent advancements in the field of artificial intelligence (AI) are based in deep learning techniques. In classic machine learning approaches the input data are manually preprocessed by humans, which is called feature engineering. These hand-designed features are the input for the artificial neural network (ANN) or any other sort of statistical model which predicts the output. The process of feature engineering can be a big effort and requires domain knowledge about the data from the application engineer. For more complex problems it is sometimes not even possible to create the features by hand, for example in the field of face recognition or speech-to-text applications where the inputs are pictures or time sequences. Deep learning has the approach to preprocess the input data by itself and abstract the features by using several layers of neural networks. Thereby, a lot of time and effort in the application process can be saved and more complex problems can be solved. A disadvantage is, that the higher amount of layers and parameters increases the computational effort \cite{goodfellow_deep_2016}. In this work, the input data are the detector data from the e1 (loop) detectors which are fed into the deep learning model. The hypothesis is that the deep learning model should abstract the relevant features by itself by using the knowledge of the spatial correlations within the road network (usage of graph attention layers). This makes this model to a \textit{geometric} deep learning model \cite{bronstein_geometric_2017}.

In this section the theoretical fundamentals about deep learning are presented, which are necessary to successfully implement geometric deep learning networks for queue length estimation. Section \ref{sec:basics_NN} starts with the basics and general introduction of feedforward neural networks. To extract spatial information from the inputs, graph attention layer is introduced in section \ref{sec:gat_layer}. Recurrent neural networks (RNNs), presented in section \ref{sec:RNN}, are used to store relevant information over multiple time steps and represent the main component for the  RNN encoder-decoder model introduced in section \ref{sec:enc-dec}.

\subsection{Basics of Feedforward Neural Networks} \label{sec:basics_NN}
 Feedforward neural networks are the most simple and fundamental kind of deep learning models.
 When it comes to solving real-world problems, neural networks have great characteristics like nonlinearity, parallelism, handling of uncertain and fuzzy information as well as the ability to generalize knowledge \cite{basheer_artificial_2000}. Generally, the aim of these models is to approximate a function $f^*$. The general formulation for a regression would be $ \boldsymbol{\hat{y}} = f(\boldsymbol{x}, \boldsymbol{W})$, where $\boldsymbol{x}$ is the input, $\boldsymbol{\hat{y}}$ the predicted output and $\boldsymbol{W}$ the weight matrix. During the training process, the optimization algorithm learns the parameters that $f$ approximates $f^*$ the best. These models are called feedforward neural networks, since the input is fed trough the network and results an output without a feedback loop. Once a feedback loop is implemented, the model is called recurrent neural network (see section \ref{sec:RNN}). 
 
 \subsubsection{Structure} \label{sec.structure}
 
 Inspired by biological neural networks, a complex artificial neural network consists of many simple elements (artificial neurons or nodes). The analogy between the biological neurons to the artificial neurons is presented in Fig. \ref{bild.neurons}.
 
 \begin{figure}[h]
 	\centering
 	\includegraphics[width=1\textwidth]{deeplearning/neuron_example.png}
 	\caption[Analogy between biologial and artificial neurons]{Analogy between biologial (left) and artificial neurons (right) \cite{basheer_artificial_2000}.} \label{bild.neurons}
 \end{figure}

At the artificial neuron, the inputs $x_1$ to $x_n$ are multiplied with the corresponding weights $w_1$ to $w_n$ and get summed-up (this process is called \textit{affine transformation}). Afterwards, the sum is an input for the activation function, which adds the nonlinearity to the model. In this particular case, the activation function is a step function, which only lets the value pass, if a threshold is reached. But there are also other functions possible (shown in Fig. \ref{bild.activation_functions}).
 \begin{figure}[h]
 	\centering
 	\includegraphics[width=1\textwidth]{deeplearning/activation_functions.png}
 	\caption[Activation functions for deep learning models]{Examples for activation functions: step-function (left), tanh function (middle) and the rectified linear unit (ReLU) function (right) \cite{neubig_neural_2017}.} \label{bild.activation_functions}
 \end{figure}
 According to \cite{goodfellow_deep_2016}, the most recommended default activation function for deep learning applications is the ReLU function, which is defined by $\sigma(z) = max\{0,z\}$. Due to its piecewise linear characteristic, it has good optimization properties for gradient-based optimization algorithms.   
 Generally, neural networks chain together many simple affine transformations and activation functions to represent more complex functions. Due to this simple structure, it is easier and more efficient to train.
 A very good example for explaining how deep neural networks in principle work, is solving the XOR problem. The visualization of the XOR problem is shown in Fig. \ref{bild.XOR_problem} on the left.
  \begin{figure}[h]
  	\centering
  	\includegraphics[width=1\textwidth]{deeplearning/XOR_problem.png}
  	\caption[The XOR problem in deep learning] {The XOR problem with the original $\boldsymbol{x}$ space of the XOR logic on the left and the transformed representation after the first hidden layer (learned $\boldsymbol{h}$ space) on the right \cite{goodfellow_deep_2016}.} \label{bild.XOR_problem}
  \end{figure}
  For the original $\boldsymbol{x}$ space of the XOR logic, it is not possible to classify between 1 and 0 just by dividing the space into two parts by a line, since there is no configuration of a line that would separate the zeros from the ones. According to the XOR logic, the value becomes only one if exactly one of the values $x_1$ or $x_2$ is one. So a basic linear model like
  
  \begin{equation}
  	y = \boldsymbol{w^T}\boldsymbol{x}+\boldsymbol{b}
  \end{equation} 
  
  with the weights $\boldsymbol{w}$ and the bias $\boldsymbol{b}$ is not able to model the XOR logic and divide the zeros from the ones. This problem can be solved by implementing a slightly more complicated structure by adding a \textit{hidden layer} and splitting the calculation in two steps.
  
  \begin{equation} \label{eq:hidden_layer}
  	\boldsymbol{h} = ReLu(\boldsymbol{W}_{xh}\boldsymbol{x}+\boldsymbol{b}_h)
  \end{equation}
  \begin{equation} \label{eq:output_layer}
  	y = \boldsymbol{w}_{hy}\boldsymbol{h}+b_y
  \end{equation}
Eq. \ref{eq:hidden_layer} represents the hidden layer which takes as inputs the vector $\boldsymbol{x}$ and outputs the vector $\boldsymbol{h}$. The transformed space $\boldsymbol{h}$ is shown in Fig. \ref{bild.XOR_problem} on the right. During the training process, the parameters $\boldsymbol{W}_{xh}$ and $\boldsymbol{b}_h$ are learned so that after the transformation it is possible to apply a linear model, which separates both patterns. This is done by the \textit{output layer} (eq. \ref{eq:output_layer}) to calculate the result $y$. In other words: The points in the $x$ space are transformed in the $h$ space by a matrix multiplication. In this new representation in the $h$ space, it is possible to separate the zeros from the ones by a line. The classification problem is solved by adding an additional hidden layer (eq. \ref{eq:hidden_layer}) to the linear model. The new structure of the model is shown in Fig. \ref{bild.XOR_structure}. 

  \begin{figure}[h]
  	\centering
  	\includegraphics[width=0.45\textwidth]{deeplearning/XOR_structure.png}
  	\caption[Structure of a model with one hidden layer] {Structure of the model to solve the XOR problem with one hidden layer. On the left side every node is drawn explicit and on the right side an simplified overview with the weights is given \cite{goodfellow_deep_2016}.} \label{bild.XOR_structure}
  \end{figure}

Generally, in a deep learning model are usually a lot more affine transformations and hidden layers so that more complex, multidimensional problems can be solved. But all this is based on very simple and easy computable affine transformations with following activation functions. So the first layer could be generally described as
\begin{equation} \label{eq:normal_NN}
	\boldsymbol{h}^{(1)} = \sigma^{(1)}(\boldsymbol{W}^{(1)}\boldsymbol{x}+\boldsymbol{b}^{(1)})
\end{equation}
with $\boldsymbol{x}$ as input and $\boldsymbol{W}^{(1)}$ as well as $\boldsymbol{b}^{(1)}$ as trainable parameters. The sum is input for the activation function $\sigma(\cdot)$. The second hidden layer is then given by
\begin{equation}
	\boldsymbol{h}^{(2)} = \sigma^{(2)}(\boldsymbol{W}^{(2)}\boldsymbol{h}^{(1)}+\boldsymbol{b}^{(2)})
\end{equation}
which takes now $\boldsymbol{h}^{(1)}$ as input. The activation functions $\sigma^{(i)}$ do not necessarily have to be the same. The next hidden layer takes $\boldsymbol{h}^{(2)}$ as input with its own weights and activation function and so on. The last layer of this series is called the \textit{output layer}. The \textit{depth} of the network is defined by number of layers that are chained together. The \textit{width} of the model is determined by the size of the outputs of the hidden layers $\boldsymbol{h}^{(i)}$.

How powerful it can be to transform the inputs into another representation is emphasized in Fig. \ref{bild.cartesian_polar}. 
  \begin{figure}[h]
  	\centering
  	\includegraphics[width=0.8\textwidth]{deeplearning/cartesian_polar_representation.png}
  	\caption[Comparison between patterns in cartesian and polar coordinates] {Comparison between patterns in cartesian and polar coordinates \cite{goodfellow_deep_2016}.} \label{bild.cartesian_polar}
  \end{figure}
Similar to the XOR-Problem, for this example it is also impossible to separate both patterns with a linear model when the representation is in cartesian coordinates. But it becomes possible once the points are transformed in polar coordinates by a hidden layer. Generally, the main task of layers in a neural network is to transform the inputs (features) into another coordinate-space, where it is possible to fulfill the original task which could be classification or linear regression. 

The optimal structure of a network with the depth, width and kind of activation functions can only be found in an experimental way, monitoring the errors for the training, test and validation set \cite{goodfellow_deep_2016}. To reach this goal, it is essential to understand the fundamentals how neural networks are trained and how optimization algorithms work. The following chapter provides a brief introduction in this field. 


\subsubsection{Training and Optimization}
%intoduce words like supervised learning, targets, freatures
Generally, neural networks are able to solve a variety of tasks, but they have to be specifically trained for this. These tasks can be for instance \textit{classification}, where the network determines the class the input data belongs to. An example would be an deep neural network which has animal pictures as input data and the task is to classify, whether in the picture is a cat, a dog or another animal. A different task would be \textit{regression}, where the output data are a  continuous graph. In this thesis, the presented neural network solves a regression problem, since it has to estimate the time sequence of the queue length based on time sequences of detector data as input. 
Another way to categorize learning algorithms is to differentiate between \textit{supervised} and \textit{unsupervised} learning. In case of machine/deep learning the input data are called \textit{features} $\boldsymbol{x}$ and the ground-truth output data are \textit{targets} or \textit{labels} $\boldsymbol{y}$. \textit{Unsupervised learning algorithms} though, use only the features for training without having corresponding targets. Usually the dataset has many features and the learning algorithm tries to learn correlations within the data. This can be used for tasks like denoising or clustering, where the dataset gets divided into several clusters containing data with similar properties .
For \textit{supervised learning algorithms} exist features $\boldsymbol{x}$ as well as corresponding targets $\boldsymbol{y}$. During training, the neural network model learns to predict $\boldsymbol{y}$ given the the input $\boldsymbol{x}$. This applies to this thesis, with the detector data as features $\boldsymbol{x}$ and the queue length as target $\boldsymbol{y}$. After training, the model should be able to predict an unknown $\boldsymbol{y}$ for a new $\boldsymbol{x}$. 
%mention briefly reinforcement learning, then introduce dataset, loss functions and then backprop
Another popular training method is \textit{reinforcement learning}, where the training model does not learn from a given dataset but from experience by interacting with an environment. But this is beyond the scope of this thesis \cite{goodfellow_deep_2016}. 

Summarized, in case of queue length estimation the approach is a regression problem which is solved by a supervised learning algorithm. For training of a deep neural network it is essential to have a large dataset, which contains of many examples with $n$ features ($\boldsymbol{x} \in \R^n$) and $m$ targets ($\boldsymbol{y} \in \R^m$). To describe the entire dataset with $k$ examples ($\boldsymbol{x}_1 ... \boldsymbol{x}_k$ and $\boldsymbol{y}_1 ... \boldsymbol{y}_k$), all of these examples are concatenated to a matrix $\boldsymbol{X} \in \R^{k \times n}$ (\textit{design matrix}) and $\boldsymbol{Y} \in \R^{k \times m}$.The symbol $k$ is called number of \textit{samples}. %now loss functions
During one training step in a supervised learning algorithm, the model gets one example $\boldsymbol{x}$ and predicts the output $\boldsymbol{\hat{y}}$. After the prediction, $\boldsymbol{\hat{y}}$ is compared to the provided ground-truth $\boldsymbol{y}$. This is usually made by \textit{loss functions}. The most common function for regression problems is the \textit{mean squared error} which is for $n$ features

\begin{equation}
	MSE = \frac{1}{n} \sum_{i=1}^{n} (\boldsymbol{\hat{y}}_i^2 - \boldsymbol{y}_i^2).
\end{equation}

If in one training step more than one example is used, the average of every single MSE is calculated. The loss determines how good the prediction is regarding the target. The goal of the training algorithm is to adjust the weights of the neural network, so that the loss gets reduced and the prediction converges to the target. Generally, to minimize the loss is a classic numerical optimization problem, which can be solved by well known numerical optimization algorithms. The most common optimization algorithms are \textit{gradient-based} algorithms. They use the derivative of the function (in this case the deep learning model represents the function) to get information about how to adjust $\boldsymbol{x}$ (or hidden states $\boldsymbol{h}$) in order to minimize the MSE between $\boldsymbol{\hat{y}}$ and $\boldsymbol{y}$. The simplest method is the \textit{gradient descent}, where $\boldsymbol{x}$ (or $\boldsymbol{h}$) is moved in the direction of the opposite sign of the derivative \cite{goodfellow_deep_2016}. 
For a successful optimization it is essential to determine the derivatives in the neural network model. 
% explain principle of back-propagation and why it is necessary. How is it implemented in computer?
In the previous subsection \ref{sec.structure} the fundamental structure is presented. It is shown, how the input $\boldsymbol{x}$ propagates trough the network and is computed, so that the output $\boldsymbol{\hat{y}}$ results. This process is called \textit{forward propagation}. During training, the forward propagation of the training data $\boldsymbol{x}$ results in the estimated output $\boldsymbol{\hat{y}}$. For convenience, the simple model from eq. \ref{eq:hidden_layer} and \ref{eq:output_layer} are shown again extended with the loss $l$ and modeled the ReLu function as a single step:

\begin{equation}
	  \begin{split} \label{eq:simple_model1}
	  \boldsymbol{h^{\prime}} &= \boldsymbol{W}_{xh}\boldsymbol{x}+\boldsymbol{b}_h \\
	  \boldsymbol{h} &= ReLu(\boldsymbol{h^{\prime}}) \\
	  \hat{y} &= \boldsymbol{w}_{hy}\boldsymbol{h}+b_y \\
	  l &= (\hat{y} - y)^2\\
	  \end{split}
\end{equation}

The derivatives of this model can be calculated by a method called \textit{back propagation}. With the chain rule the derivatives can be calculated for every set of weights. 

\begin{equation}
\begin{split} \label{eq:derivatives}
	\frac{dl}{db_y} &= \frac{dl}{d\hat{y}}\frac{d\hat{y}}{db_y} \\	
	\frac{dl}{d\boldsymbol{w}_{hy}} &= \frac{dl}{d\hat{y}}\frac{d\hat{y}}{d\boldsymbol{w}_{hy}} \\	
	\frac{dl}{d\boldsymbol{b}_h} &= \frac{dl}{d\hat{y}}\frac{d\hat{y}}{d\boldsymbol{h}}\frac{d\boldsymbol{h}}{d\boldsymbol{h^{\prime}}}\frac{d\boldsymbol{h^{\prime}}}{d\boldsymbol{b}_h} \\	
	\frac{dl}{d\boldsymbol{W}_{xh}} &= \frac{dl}{d\hat{y}}\frac{d\hat{y}}{d\boldsymbol{h}}\frac{d\boldsymbol{h}}{d\boldsymbol{h^{\prime}}}\frac{d\boldsymbol{h^{\prime}}}{d\boldsymbol{W}_{xh}} \\	
\end{split}
\end{equation}

In eq. \ref{eq:derivatives} the derivatives for all the weights regarding the loss function are presented. The chain rule allows to calculate the derivatives for every single step in the back propagation and multiply the results to get the derivatives for every single weight.
The derivations can become very complicated for larger networks so that it is impossible to calculate them by hand. Fortunately, it is possible to let the computer calculate the derivatives by using \textit{automatic differentiation (autodiff)}, where the feedforward propagation is modeled in many single steps (e.g addition, multiplication, square, ...) and the single derivatives are computed. So it is possible to create large networks and provide for every single neuron the forward function and the backward derivative computation \cite{neubig_neural_2017}.  

Once the forward propagation and the derivatives can be provided, the numerical gradient-based optimization algorithm is able to adjust the weights and minimize the loss. 
The fundamental form of the gradient descent algorithm is 
\begin{equation}
	\boldsymbol{x^{\prime}} = \boldsymbol{x} - \epsilon\boldsymbol{\nabla}_{\boldsymbol{x}}f(\boldsymbol{x})
\end{equation}

where $\boldsymbol{x^{\prime}}$ is the new approximation for the minimum, $\epsilon$ is the \textit{learning rate} and $\boldsymbol{\nabla}_{\boldsymbol{x}}f(\boldsymbol{x})$ is the gradient of $f$ which contains the partial derivatives. The learning rate is a fundamental \textit{hyperparameter}. Hyperparameters are parameters which control the learning algorithm. Further down in this section a few more will be introduced. 
The learning rate is important, since it has high influence on the training algorithm. If $\epsilon$ is too low, it takes a lot of training steps to reach the global minimum, which is highly inefficient. Furthermore it is possible, that the algorithm only finds a local minimum but not a global. Multidimensional optimization problems often have more than one minimum. This is visualized for a simple one dimensional case in fig. \ref{bild.multiple_minima}.

\begin{figure}[h]
  	\centering
  	\includegraphics[width=0.8\textwidth]{deeplearning/multiple_minima_plot.png}
  	\caption[Multiple minima in an optimization problem] {Multiple minima in an optimization problem \cite{goodfellow_deep_2016}.} \label{bild.multiple_minima}
\end{figure}

 If the learning rate is too high, it is possible that the algorithm cannot find a acceptable minimum either, since the algorithm "jumps" over the minimum. 
 The probably most common and used optimization algorithm for machine and deep learning is \textit{stochastic gradient descent} (SGD), which is a modification of the gradient descent method. Instead of computing the gradient based on only one example, SGD uses a minibatch of multiple examples to compute the average gradient. This results in a better generalization of the knowledge, since more parallel information are taken into consideration. Addressing the problem of the right choice of the learning rate, algorithms with adaptive learning rates have been developed. The most important in the field of deep learning are \textit{AdaGrad}, \textit{RMSProp} and \textit{Adam}. To present the algorithms in detail is beyond the scope of this thesis. \cite{goodfellow_deep_2016} gives a good overview of this topic. 
%show graphic with nice optimization algorithm and stepsize and so on... (implement maybe later, but no musthave!)

One of the main challenges when it comes to train neural networks is the phenomenon of \textit{underfitting} and \textit{overfitting}. Before training the model, the entire dataset is split into the \textit{training data} and \textit{test data}. The model is trained with the training data and afterwards the \textit{training loss} can be calculated. Furthermore, the model is tested on the test data it has never seen before during training. For the test session, the tests loss could be calculated as well. The ability of a model to make good predictions on data it has never observed before is called \textit{generalization}. The losses for training and testing over the \textit{model capacity} is shown in fig. \ref{bild.Loss_over_capacity} for a specific problem, which is not trivial but also not too complex. 
\begin{figure}[h]
	\centering
	\includegraphics[width=1\textwidth]{deeplearning/Loss_over_capacity.png}
	\caption[Underfitting and overfitting regarding model capacity] {Underfitting and overfitting regarding model capacity \cite{goodfellow_deep_2016}.} \label{bild.Loss_over_capacity}
\end{figure}
Simplified, the model capacity describes the complexity of the model regarding the number of hidden layers, the width and other structural properties. Models with a low capacity are not able to solve more complex problems. This leads to underfitting, where the training loss as well as the test loss is very high. The model cannot generalize knowledge, since it cannot even learn the information provided by the training data. Overfitting occurs if the model capacity is too high for the complexity of the given problem. The model has enough parameter to learn the whole training set, which results in a low training loss. The test loss is high though, because the model memorizes learned properties from the individual test data, which are not relevant for solving the problem. 
\begin{figure}[H]
	\centering
	\includegraphics[width=0.6\textwidth]{deeplearning/graph_under_overfitting.png}
	\caption[Visualization of the impact of underfitting and overfitting] {Visualization of the impact of underfitting and overfitting \cite{basheer_artificial_2000}.} \label{bild.under_overfitting}
\end{figure}
In this case, the model cannot generalize the knowledge either. This phenomenon is presented in detail in fig. \ref{bild.under_overfitting}.
For easier understanding of the figure, the model can be interpreted as a polynomial function. If the model complexity is too low (in this case polynomial of order one), the curve cannot fit the training points and also fails for an accurate prediction of the test points (both training and test loss are high). This is the classic case of underfitting. When the model complexity is increased to a polynomial function of second order, it fits quiet well for the training data but still has a rest loss, which is not zero. It also has a low loss for the test points, which is in this case the optimal solution. If the order of the polynomial increases even more (e.g order nine), the curve fits trough all the training points and the training loss is zero. But when it comes to predict the test points, the graph does not fit anymore and the test loss is very high. Then the model is overfitted. 

It is crucial to find the optimal model capacity to avoid underfitting or overfitting. The necessary complexity of the model highly depends on the individual problem to be solved. So there is no other way than using the trial-and-error method and maybe having experience from other applications. In addition to that, it is also possible (and recommended) to use regularization techniques during the training. Regularization has the aim to avoid overfitting and reduce the test loss on cost of an increasing train loss. In this section, only two (for this thesis relevant) regularization methods are briefly introduced. The first is \textit{parameter norm penalties}, in particular the $L^2$ \textit{parameter regularization}. 
\begin{figure}[H]
	\centering
	\includegraphics[width=0.6\textwidth]{deeplearning/L2_regularization.png}
	\caption[Visulaization of the $L^2$ regularization] {Visualization of the $L^2$ regularization \cite{goodfellow_deep_2016}. The point $\boldsymbol{w}^*$ represents the optimal parameter $w_1$ and $w_2$ to fit the training data. The dotted circles represent the increasing value of the penalty term with increasing distance to the origin. The optimum can be found in the point $\tilde{\boldsymbol{w}}$}. \label{bild.L2_regularization}
\end{figure}
Generally, for parameter regularization a penalty term is added to the loss functions which contains the weights $\boldsymbol{W}$ of each hidden layer. In case of the $L^2$ regularization the penalty term is $\Omega = \frac{1}{2} \lVert \boldsymbol{W} \rVert_2^2$. This additional term reduces high weights and overfitting to a particular training set. This method is also called \textit{weight decay}. 
In fig. \ref{bild.L2_regularization} the influence of the parameter regularization is presented.
Shown are the weights $\boldsymbol{w}^*$ which represents the parameter which would optimal fit the training dataset. The ellipses around this point visualize the increasing loss function without the penalty term for the parameter $w_1$ and $w_2$. The dotted circles represent the increasing value of the penalty term based on $w_1$ and $w_2$. The optimum between both the ellipses and dotted circles can be found in the point $\tilde{\boldsymbol{w}}$. In this way the $L^2$ regularization avoids the overfitting of the parameters to the point $\boldsymbol{w}^*$.
Another common regularization technique is \textit{dropout}. When dropout is applied during training, some weights are randomly set to zero. This creates a subnetwork of the original neural network which is then trained. In the next training step other weights are randomly chosen to be set to zero. This technique reduces on the one hand the capacity of the model which results in a need for higher number of nodes which requires more computational effort. On the other hand it reduces overfitting, since the structure of the neural network changes slightly in every training step. 

%\begin{equation}
%	\forall \; simulation, \forall \; timestep < t
%\end{equation}

The here briefly presented methods are fundamental for creating and training a deep learning model. However, deep learning is a large topic with many different applications and methods. A very good overview and introduction gives \cite{goodfellow_deep_2016}. In this thesis the focus in the following sections is on attention mechanisms and sequence to sequence problems in deep learning. Since in this approach the model uses data which have spatial correlations (lanes are connected to each other), it is beneficial to use attention mechanisms to let the model focus on relevant information.


\subsection{Graph Attention Networks} \label{sec:gat_layer}
The here presented \textit{graph attention networks} are designed to perform on geometric graphs which consist of \textit{nodes} and \textit{edges}. Each node is connected with other nodes by edges. Examples for graphs are social networks, road networks or 3D meshes. The structure does not necessarily have to be a grid-like structure. 
For solving tasks where it is possible to model correlations between data in a graph structure, it is often helpful to consider not only a single node, but its neighboring nodes. If the algorithm uses deep learning attention mechanisms for that, this process is called \textit{graph attention}. In this section a new method for learning attention for a graph, based on \cite{velickovic_graph_2017}, is presented. Described is a single \textit{graph attentional layer (GAT)}, which can be used to build larger graph attention networks. The input for this layer is a matrix which consists of every node of the graph including its features $\boldsymbol{h}_i$

\begin{equation}
	\boldsymbol{H} = \{\boldsymbol{h}_1,\boldsymbol{h}_2,...,\boldsymbol{h}_N\},\boldsymbol{h}_i \in \R^F, \boldsymbol{H} \in \R^{N \times F}.
\end{equation}

where $N$ is the number of nodes and $F$ is the number of features. The second input for the GAT layer is the information about the connections of the nodes in the graph. It is represented by the \textit{adjacency matrix}

\begin{equation}
	\boldsymbol{A} \in \{0, 1\}^{N \times N}.
\end{equation}

$\boldsymbol{A}$ is a binary matrix with the size number of nodes by number of nodes. If a node has a connection to another node, the value at this specific place in the matrix is one, otherwise it is zero. Before computing the output features for every node, it is necessary to compute \textit{attention coefficients} $e_{ij}$ for every node $i$ and its corresponding neighbors $j$ in the \textit{neighborhood} $\mathcal{N}_i$. The neighborhood $\forall \boldsymbol{h}_i: \mathcal{N}_i$ can be extracted by using the adjacency matrix. The single attention coefficients are calculated by

\begin{equation}
	e_{ij} = \sigma (\boldsymbol{a}^T [\boldsymbol{Wh}_i \lVert \boldsymbol{Wh}_j])
\end{equation}

with the \textit{weight matrix} $\boldsymbol{W} \in \R^{F^{\prime} \times F}$, where $F^{\prime}$ is the number of the new output features, and a \textit{weight vector} $\boldsymbol{a} \in \R^{2F^{\prime}}$. Furthermore, the $\lVert$ symbol represents the concatenation of the results of both matrix multiplications $\boldsymbol{Wh}_i$ for the node itself and $\boldsymbol{Wh}_j$ for the neighboring node. Afterwards the attention coefficients are normalized by a \textit{softmax} function, which allows a comparison between the coefficients:

\begin{equation}
\alpha_{ij} = \frac{exp(e_{ij})}{\sum_{k \in \mathcal{N}_i} exp(e_{ik})}.
\end{equation}

After the normalization, it is possible to calculate the new hidden state of the node $i$ by executing one learnable linear transformation and weighting it with the normalized attention coefficient for every node in the neighborhood of the node (including the node itself):

\begin{equation}
\boldsymbol{h}^{\prime}_i = \sigma \Big( \sum_{j \in \mathcal{N}_i} \alpha_{ij} \boldsymbol{Wh}_j  \Big) ; \quad \boldsymbol{h}^{\prime}_i \in \R^{F^{\prime}}
\end{equation}

Generally, the normalized attention coefficient $\alpha_{ij}$ decides, how much the former features from node $j$ contributes to the new hidden state $\boldsymbol{h}_i^{\prime}$ of node $i$. 

\begin{figure}[h]
	\centering
	\includegraphics[width=0.65\textwidth]{deeplearning/pic_attn_heads.pdf}
	\caption[Visualization of graph attention mechanism with tree attention heads] {Visualization of graph attention mechanism with three attention heads \cite{velickovic_graph_2017}.} \label{bild.annt_mechanism}
\end{figure}

Furthermore, \cite{velickovic_graph_2017} notes that it can be helpful to execute the calculation of attention coefficients and new hidden states multiple times independently from each other. By that the attention learning process can be more stabilized. This is then called "\textit{multi-head attention}" \cite{velickovic_graph_2017}. After the execution of $K$ different independent estimations with the attention mechanism, one way to process the results is to concatenate them:

%formula concatenating
\begin{equation}
\boldsymbol{h}^{\prime}_i = \overset{K}{\underset {k=1}{\lVert}} \;
\sigma \Big( \sum_{j \in \mathcal{N}_i} \alpha_{ij}^k \boldsymbol{W}^k\boldsymbol{h}_j  \Big); \quad \boldsymbol{h}^{\prime}_i \in \R^{F^{\prime}}
\end{equation}

where $k$ stands for each single attention head. Also each independent attention mechanism has its own attention coefficients $\alpha_{ij}^k$ and weight matrix $\boldsymbol{W}^k$. When using concatenation of the single results, the final number of features will be $KF^{\prime}$ instead of $F^{\prime}$. Another option to process the single results from each attention head is to average over $K$

%formula averaging
\begin{equation}
\boldsymbol{h}^{\prime}_i = 
\sigma \Big( \frac{1}{K} \sum_{k=1}^{K} \sum_{j \in \mathcal{N}_i} \alpha_{ij}^k \boldsymbol{W}^k\boldsymbol{h}_j  \Big); \quad \boldsymbol{h}^{\prime}_i \in \R^{KF^{\prime}}
\end{equation}

where all the single results are summed-up and divided by the number of attention heads. In this case, the number of output features per node is $F^{\prime}$.
In fig. \ref{bild.annt_mechanism} a visualization of the attention mechanism with three attention heads is presented. In this picture $\boldsymbol{h}_1$ are the old features of node one, while $\boldsymbol{h}_2$ to $\boldsymbol{h}_6$ are the neighboring nodes. Each of them contributes, scaled by the attention coefficients $\boldsymbol{\alpha}_{1j}$, to the new hidden state $\boldsymbol{h}_1^{\prime}$. The different parallel attention heads are visualized by the colored arrows. 
Finally, the output of the GAT layer is a matrix which contains all the features for each node in the graph:

\begin{equation}
	\boldsymbol{H}^{\prime} = \{\boldsymbol{h}_1^{\prime},\boldsymbol{h}_2^{\prime},...,\boldsymbol{h}_N^{\prime}\},\boldsymbol{h}_i^{\prime} \in \R^{F^{\prime}}, \boldsymbol{H}^{\prime} \in \R^{N \times F^{\prime}}
\end{equation}

Based on the presented single GAT layer, more complex networks can be build by using more than one graph attention layer in a network. 
%Specifically for solving the problem of queue length estimation, the GAT layer can help to take traffic data from other connected lanes into consideration. This can help to make the estimation more accurate. 

\subsection{Recurrent Neural Networks (RNN)} \label{sec:RNN}

All networks that have been presented in the previous chapters were feedforward neural networks. The information from the input propagates through the network and generates an output. Every new sample as input for the deep learning model is independent from the previous or following one. Also the order of the input-examples is mostly not very relevant. 
This becomes different when the input changes to sequences. 

Sequences can be for instance sentences (sequence of words) and the task is to translate this sequence into another language. So the input is a sequence and the output is a sequence as well. The models which are used to solve this task are called \textit{sequence-to-sequence (seq2seq) models} \cite{neubig_neural_2017}. Another example are time sequences, like in the approach which is made in this thesis. The input is a time sequence of loop-detector data and the output is the queue length in form of a time sequence as well. In the case of sequences, the single steps of the sequence are not independent from each other anymore but correlated to each other. For example in the sentence "\textit{He} loves \textit{his} red bike", the third word "his" is correlated to the first word "He". It matches regarding the gender. So a deep learning model structure is necessary which reads in every single step, but does not treat them independently, but as a sequence. Therefore, \textit{recurrent neural networks (RNN)} were developed, which are able to process sequential data. These family of networks have an internal feedback loop, where the calculated hidden state $\boldsymbol{h}_{i-1}$ from the previous step is fed back as an input of the model to calculate the new hidden state $\boldsymbol{h}_i$ for the current step. This allows the network to take also information from previous steps into consideration. In fig. \ref{bild.RNN_unfold} the general topology of a RNN is presented. 

\begin{figure}[h]
	\centering
	\includegraphics[width=1\textwidth]{deeplearning/RNN_unrolled.pdf}
	\caption[Unfold RNN] {Circuit diagram of the RNN (right) and its unfolded visualization (left) after  \cite{goodfellow_deep_2016}.} \label{bild.RNN_unfold}
\end{figure}

On the left site, the circuit diagram of the RNN is presented, where for the time step $i$ the RNN has as input $\boldsymbol{x}_i$ as well as the previous hidden state $\boldsymbol{h}_{i-1}$. In this case the RNN has no other output than its hidden state, but it is also possible to add another layer to compute an output. This is presented later in section \ref{sec:enc-dec}. On the right side, the unfold visualization with every time step is presented. It is important to note, that the recurrent neural network is for every time step the same with the same weights \cite{goodfellow_deep_2016}. 
The general equation to calculate the new hidden state is

\begin{equation}
	\boldsymbol{h}_i = \sigma(\boldsymbol{W}_{xh} \boldsymbol{x}_i + \boldsymbol{W}_{hh}\boldsymbol{h}_{i-1}+\boldsymbol{b}_h).
\end{equation}

The only difference between a normal feedforward neural network (see eq. \ref{eq:normal_NN}) and a recurrent neural network is the term $\boldsymbol{W}_{hh}\boldsymbol{h}_{i-1}$. The first hidden state $\boldsymbol{h}_0$ has to be initialized, which is usually a vector of zeros. The reason why recurrent neural networks can deal with long distance dependencies is, that all relevant information of previous time steps are stored in the hidden state $\boldsymbol{h}_{i-1}$ \cite{neubig_neural_2017}. 

The presented structure above is very simple and a straight forward development from a feedforward neural network. However, it has limitations due to the \textit{vanishing gradient} or \textit{exploding gradient} problem. The procedure to train a RNN is the same than for a normal neural network, which includes the forward propagation based on the input and following the back propagation using the gradients to optimize the weights. But in case of a RNN, the back propagation includes all previous time steps of the input sequence. If $\frac{d\boldsymbol{h}_{i-1}}{d\boldsymbol{h}_i}$ is not exactly one, the gradient between the hidden state at time step $i$ and the loss function $\frac{dl}{d\boldsymbol{h}_i}$ becomes either very small or very large. That means for a very long sequence, it is possible that the gradient at the beginning of the sequence is too small to have an effect to update the weights. 
The most popular solution for solving the vanishing and exploding gradient problem was introduced by \cite{hochreiter_long_1997} in 1997 and called \textit{long-short-term-memory (LSTM)}. It uses parallel to the hidden state $\boldsymbol{h}_i$ a \textit{memory cell} $\boldsymbol{c}$ which long and short term dependencies can be stored. Since $\frac{d\boldsymbol{c}_{i-1}}{d\boldsymbol{c}_i}$ is exactly one, no vanishing or exploding of the gradients occur. The LSTM can control which knowledge to keep in the memory cell and which knowledge to delete by using so called \textit{gates}. It uses \textit{input} and \textit{output} \textit{gates}, which both consist of an affine transformation with a following activation function. So the LSTM can learn, how to manage the information and which knowledge to keep over time and which not. LSTM had great success in solving seq2seq problems during the past years \cite{neubig_neural_2017}. 
However, in this thesis another variation of a recurrent neural network, which is called \textit{gated recurrent unit (GRU)}, will be used. It was first presented in \cite{cho_learning_2014} in 2014 and can be described as a simplification of an LSTM. It has no memory cell $\boldsymbol{c}$ but only uses the hidden state $\boldsymbol{h}$ for storing long term dependencies. It also has only two gates which are the \textit{update gate} $\boldsymbol{z}$ and the \textit{reset gate} $\boldsymbol{r}$. Although it is a simplification, the performance regarding sequence processing can be similar to an LSTM \cite{chung_empirical_2014}. The main structure is presented in fig. \ref{bild.GRU}. 

\begin{figure}[h]
	\centering
	\includegraphics[width=1\textwidth]{deeplearning/GRU.pdf}
	\caption[Visualization of a gated recurrent unit (GRU)] {Visualization of a gated recurrent unit (GRU) with the reset gate $\boldsymbol{r}$, update gate $\boldsymbol{z}$ and proposal hidden state $\boldsymbol{\tilde{h}}$ after  \cite{cho_learning_2014}. } \label{bild.GRU}
\end{figure}

The hidden state from the previous time step $\boldsymbol{h}_{i-1}$ as well as the current time step from the input sequence $\boldsymbol{x}_i$ are fed into the GRU. The first step is to calculate the proposed new hidden state

% calculate new proposal state
\begin{equation}
\boldsymbol{\tilde{h}}_i = tanh(\boldsymbol{Wx}_i+\boldsymbol{U}[\boldsymbol{r}_i \circ \boldsymbol{h}_{i-1}]+\boldsymbol{b})
\end{equation}

by using $\boldsymbol{h}_{t-1}$ and $\boldsymbol{x}_i$. The input $\boldsymbol{x}_i$ is multiplied with the weight matrix $\boldsymbol{W}$. Furthermore, $\boldsymbol{U}$ weights the element-wise multiplication ($\circ$) between the reset gate $\boldsymbol{r}_i$ and $\boldsymbol{h}_{i-1}$. The reset gate controls, which information of the previous hidden state contributes to the proposal state. The reset gate can be calculated as

%reset gate r_i
\begin{equation}
\boldsymbol{r}_i = \sigma (\boldsymbol{W}_r \boldsymbol{x}_i + \boldsymbol{U}_r \boldsymbol{h}_{i-1}+ \boldsymbol{b}_r).
\end{equation}

The calculation of the new hidden state is

%update new hidden state
\begin{equation}
\boldsymbol{h}_i = (1-\boldsymbol{z}_i)\circ \boldsymbol{h}_{i-1}+\boldsymbol{z}_i \circ \boldsymbol{\tilde{h}}_i; \quad \boldsymbol{h}_0 = \boldsymbol{0}
\end{equation}

where the update gate determines the ratio between the contribution of the previous and the proposal hidden state. The update gate can be calculated as

% update gate z_i
\begin{equation}
\boldsymbol{z}_i = \sigma (\boldsymbol{W}_z \boldsymbol{x}_i + \boldsymbol{U}_z \boldsymbol{h}_{i-1} + \boldsymbol{b}_z)
\end{equation}

with the weight matrices $\boldsymbol{W}_z$ and $\boldsymbol{U}_z$. Due to this structure, the GRU is able to solve tasks with long time dependencies in a sequence and still having a quiet simple model complexity \cite{cho_learning_2014}\cite{bahdanau_neural_2014}. Gated recurrent units are the main component for the processing sequences with an encoder-decoder structure, which is presented in the following section.
 

\subsection{RNN Encoder-Decoder} \label{sec:enc-dec}

The best approach to solve sequence-to-sequence models, is to use an \textit{RNN Encoder-Decoder} structure. Generally, two recurrent neural networks are sequentially used. The first RNN is the encoder, which gets a sequence as input and encodes it into hidden states. The decoder maps the information in the hidden states back into the output sequence. This algorithm is presented in \cite{cho_learning_2014}. In this thesis both RNN, the encoder and decoder, are GRU. In addition to that, in this thesis an \textit{attention decoder} based on \cite{bahdanau_neural_2014} is used. The attention mechanism is supposed to learn temporal attention within the time sequence. The main structure of the Encoder-Attention Decoder is presented in fig. \ref{bild.RNN_enc_dec}.

\begin{figure}[h]
	\centering
	\includegraphics[width=1\textwidth]{deeplearning/Encoder_Decoder_variant.pdf}
	\caption[Main structure of the RNN Encoder-Attention Decoder] {Main structure of the RNN Encoder-Attention Decoder in unfolded visualization. The encoder is presented in green, the attention mechanism in red and the decoder in blue \cite{cho_learning_2014}. } \label{bild.RNN_enc_dec}
\end{figure}

The encoder takes the input sequence $\boldsymbol{x}_1...\boldsymbol{x}_T$ and encodes it into hidden states for every time step. This process is equal to the GRU presented in the previous section \ref{sec:RNN}. The hidden state $\boldsymbol{h}_i$ has information about the current and all the previous inputs. The initial state $\boldsymbol{h}_0$ is chosen to a vector of zeros. 
The attention mechanism takes all the hidden states from the previous and current time step $\boldsymbol{h}_1 ... \boldsymbol{h}_i$ as well as the previous hidden state from the decoder $\boldsymbol{s}_{i-1}$ and calculates the \textit{context vector} $\boldsymbol{c}_i$ for every time step as

%context vector
\begin{equation}
	\boldsymbol{c}_i = \sum_{j=1}^{i}\alpha_{ij}\boldsymbol{h}_j
\end{equation}

with the normalized attention coefficients $\alpha_{ij}$ for every previous and the current time step $1...i$ regarding the current time step $i$. In the convex combination $\alpha_{ij}$ decides, how much the hidden state from each time step contributes to the calculation of the new output by the decoder. The original source \cite{bahdanau_neural_2014} takes all hidden states from all time steps (past and future) into consideration, since the original application is in the field of language translation, where the full sequence is already known in advance. In this case, the attention mechanism takes only the time steps from the past into consideration, since it is a time sequence and the future time steps are unknown. 
The normalized attention coefficients are calculated as 

%normalization of attention coefficients
\begin{equation}
\alpha_{ij} = \frac{exp(e_{ij})}{\sum_{k=1}^{T} exp(e_{ik})}
\end{equation}
with the attention coefficients
%attention coefficients
\begin{equation}
e_{ij} = \boldsymbol{v}_a^T tanh(\boldsymbol{W}_a \boldsymbol{s}_{i-1} + \boldsymbol{U}_a \boldsymbol{h}_j).
\end{equation}

The previous hidden state from the decoder $\boldsymbol{s}_{i-1}$ is multiplied by the weight matrix $\boldsymbol{W}_a$ and the the hidden state at time step $j$ from the encoder is multiplied by $\boldsymbol{U}_a$. After applying a $tanh$ function as activation function, the vector $\boldsymbol{v}_a$ scales the term down to a scalar which results in the attention coefficient $e_{ij}$. Note that this attention mechanism is similar to the spatial attention for the GAT layer in section \ref{sec:gat_layer}. 

Now the sequnce is encoded into hidden states and the attention mechanism selects the relevant hidden states from the past time steps. The decoder, which consists also of an GRU, takes the context vector $\boldsymbol{c}_i$ in each time step and calculates, based on the previous hidden state $\boldsymbol{s}_{i-1}$ and the previous output $\boldsymbol{y}_{i-1}$, the new hidden state $\boldsymbol{s}_{i}$ and the current output $\boldsymbol{y}_{i}$. Generally, the decoder has the same structure as the encoder. The new hidden state is calculated as

\begin{equation}
	\boldsymbol{s}_i = (1-\boldsymbol{z}_i) \circ \boldsymbol{s}_{i-1} + \boldsymbol{z}_i \circ \boldsymbol{\tilde{s}}_i
\end{equation}
where the proposal hidden state, the update gate and the reset gate are calculated as
\begin{equation}
	\begin{split}
	\boldsymbol{\tilde{s}}_i =& tanh(\boldsymbol{W}^{\prime} \boldsymbol{y}_{i-1} + \boldsymbol{U}^{\prime} [\boldsymbol{r}_i \circ \boldsymbol{s}_{i-1}] + \boldsymbol{C}^{\prime} \boldsymbol{c}_i + \boldsymbol{b}^{\prime}) \\
	\boldsymbol{z}_i = &\sigma(\boldsymbol{W}_z^{\prime} \boldsymbol{y}_{i-1} + \boldsymbol{U}_z^{\prime} \boldsymbol{s}_{i-1} + \boldsymbol{C}_z^{\prime} \boldsymbol{c}_i + \boldsymbol{b}_z^{\prime}) \\
	\boldsymbol{r}_i = &\sigma(\boldsymbol{W}_r^{\prime} \boldsymbol{y}_{i-1} + \boldsymbol{U}_r^{\prime} \boldsymbol{s}_{i-1} + \boldsymbol{C}_r^{\prime} \boldsymbol{c}_i + \boldsymbol{b}_r^{\prime}).
	\end{split}
\end{equation}

The notation $(\cdot)^{\prime}$ at the weight matrices means, that these are different to the weight matrices for the encoder in section \ref{sec:RNN}. Furthermore, the context vector $\boldsymbol{c}$ is taken into consideration and weighted by the matrices $\boldsymbol{C}^{\prime}$, $\boldsymbol{C}_z^{\prime}$ and $\boldsymbol{C}_r^{\prime}$. The initial input vector $\boldsymbol{y}_0$ is set to a zero-vector. The initial hidden state for the decoder is determined as $\boldsymbol{s}_0 = tanh(\boldsymbol{W}_s^{\prime} \boldsymbol{h}_1)$, where $\boldsymbol{W}_s^{\prime}$ is a trainable weight matrix. Except of this modification the calculation of the new hidden state is similar to the presented GRU in section \ref{sec:RNN}. To calculate the output for the specific time step $i$, the decoder GRU is extended with a single output layer:

\begin{equation}
	\boldsymbol{y}_i = \sigma(\boldsymbol{W}_o^{\prime} \boldsymbol{y}_{i-1} + \boldsymbol{U}_o^{\prime} \boldsymbol{s}_{i-1} + \boldsymbol{C}_o^{\prime} \boldsymbol{c}_i + \boldsymbol{b}_o).
\end{equation}

This layer computes, based on the previous output $\boldsymbol{y}_{i-1}$, hidden state $\boldsymbol{s}_{i-1}$ and current context vector $\boldsymbol{c}$ the current output for time step $i$ which is part of the output sequence \cite{bahdanau_neural_2014}.

In this chapter the basics of feedforward and recurrent neural networks as well as the RNN encoder-decoder algorithm is presented. Based on this methods, it is possible to create an approach for solving the task of queue length estimation in road networks. Also the presented attention mechanisms for spatial correlation (see GAT layer in section \ref{sec:gat_layer}) and temporal correlations in the sequence (this section) help to be potential superior to classic approaches like the method after \cite{liu_real-time_2009} presented in chapter \ref{sec.liu_method}.


\section{Implementation} \label{sec.DL_implementation}

The theoretical background for implementing the deep learning model was presented in the previous section. In this section, the focus is on the implementation of these methods to create a deep learning model in the programming language Python. Furthermore, the procedure for generating the dataset, which is used for training, validation and testing, is presented.

There has been a lot of progress in the recent years regarding software tools, which are developed to simplify the implementation of powerful deep learning applications. The most common software library in Python, which is used in the field of deep learning, is \textit{Tensorflow} \cite{martin_abadi_tensorflow:_2015}. It is an open source software library which is developed to perform numerical computation on a wide range of platforms (e.g. CPUs and GPUs on desktop computers but also on server clusters). It was originally developed by the Google Brain Team and became open source in 2015. Another important Python software library in this field is \textit{Keras} \cite{chollet_keras_2015}. The goal of Keras is to provide a high-level API (application program interface), which simplifies the implementation of machine learning and deep learning solutions even more. With Keras it is possible to prototype solutions very fast and generate early results. The focus of Keras is on user friendliness, modularity and easy extensibility by custom layers. Keras works on top of other, more fundamental, deep learning libraries like Tensorflow or Theano. In this thesis, the high-level API Keras is used with Tensorflow as backend. That means, all the code written with Keras is converted to Tensorflow code, which runs then as Python code on the CPU or GPU. 
 
Another important part of the implementation is to create a graph, which is an abstract representation of the road network topology. The knowledge about the graph is crucial for the graph attention layer used in the deep learning model. Fortunately, SUMO is able to export the structure of the road network as a graph using the open source Python library \textit{NetworkX} \cite{hagberg_exploring_2008}. In NetworkX it is possible to have an abstract representation of the road network as a NetworkX-graph which consists of nodes and edges. The nodes are the lanes, since they are the objects of interests with information about traffic. The lanes are connected by intersections, so in this case the intersections are represented by edges. This method of abstraction is visualized in fig. \ref{bild.NetworkX}.

%create figure which is similar to the poster from Matt
\begin{figure}[H]
	\centering
	\includegraphics[width=1\textwidth]{deeplearning/networkX.pdf}
	\caption[Abstracting graph with nodes and edges from rod network] {Abstracting graph with nodes and edges from road network; (a) represents the classic road network in SUMO; (b) visualizes the graph representation with nodes and edges \cite{wright_geometric_2018}. } \label{bild.NetworkX}
\end{figure}

On the right side (a), the classic road network with only one lane for each direction (to keep it simple) is presented. Each lane represents a node with a certain number from 1 to 8. These lanes are connected by the intersection. The figure (b) visualizes the abstracted graph representation for this example intersection. The ellipses represent the nodes (lanes with each number) which are connected by edges (straight lines). For instance cars that arrive on lane 1 in figure (a): They can leave the intersection either on lane 8 (right turn), lane 6 (straight) or lane 4 (left turn). Looking at figure (b), the node 1 is connected by arrows to node 8, 6 and 4. In this particular case it is a \textit{directed graph}, since the edges have a direction (e.g. cars can only change from lane 1 to 8 but not vice versa). If the edges do not have a certain direction, it is called an \textit{undirected graph}. The library NetworkX provides a function to abstract the adjacency matrix from the graph. In case of the example in fig. \ref{bild.NetworkX}, the adjacency matrix would be
\begin{equation}
	A =  \begin{pmatrix} 
	0 & 0 & 0 & 1 & 0 & 1 & 0 & 1 \\
	0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
	0 & 1 & 0 & 0 & 0 & 1 & 0 & 1 \\
	0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
	0 & 1 & 0 & 1 & 0 & 0 & 0 & 1 \\
	0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
	0 & 1 & 0 & 1 & 0 & 1 & 0 & 0 \\
	0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 
	\end{pmatrix}.
\end{equation}

For the usage in the graph attention layer, it is necessary to add the presented adjacency matrix to an identity matrix of the same size, so that the main diagonal of the matrix are ones. Just by that, each lane is able to consider also its own features as input rather than just its neighbors. Of course for larger road networks, like in this thesis, the road networks have more lanes and the adjacency matrix $A$ becomes larger. Especially for this thesis, $A$ includes the upstream and downstream connections of each lane, but not the neighboring lanes which are eligible for lane changing. So this is a good point to start, since the complexity of the adjacency matrix is not too high. The calculated adjacency matrix is then an input for the GAT layer and does not change over time. This is how the spatial structure of the road network is provided to the deep learning model.

The other very important input for the deep learning model are the features. In this particular approach, eight input features for each lane for every time step are used. The first six features come from the e1-detectors in SUMO, which include the \textit{number of contributed vehicles}, \textit{occupancy} and the \textit{speed} of the vehicles for the stop bar and the advanced detector. The e1 detectors provide the data for every second. The seventh input is the information about the traffic light signal at the end of the lane. It is a second-by-second binary signal which is one, if the traffic light is green and zero otherwise. The eighth feature is the estimation results of the method after \cite{liu_real-time_2009} presented in chapter \ref{sec.liu_method}. Although the estimation of this method is not accurate on larger road networks due to lane changing and stop an go traffic, it can help to guide the estimation in the right direction. The information provided by this method is just the maximum queue length for an entire traffic light cycle. Therefore, it is necessary to process a linear interpolation between the maximum length, to create second-by-second data as well.
Once, the second-by-second data for the whole simulation for every lane are collected, the features have to be gathered in a design matrix $\boldsymbol{X}$. The design matrix is assembled to the shape $[simulations \times timesteps \times lanes \times features]$. Generally, this is an array of four dimensions, where the features for each time step are collected for each lane and put together in a two dimensional matrix. In the deep learning field a four dimensional vector is also often called a \textit{tensor}. Furthermore, this is done for every time step of the simulation, which yields the third dimension. Finally, data from multiple simulations can be fed into the network, which results then in the fourth dimension. 
The same procedure can be executed for building the $Y$ array, which has the same structure except of replacing the features with the targets. In this approach the number of targets is two. The first target is the maximum queue length measured by the e2-detector in SUMO. The algorithm gives us the ground-truth data of the maximum queue length for each traffic light cycle. To get second-by-second data, a linear interpolation has to be made between the data points. The second target is the number of vehicles that are on the entire lane, and it is not relevant if they are part of the queue or not. These data can be provided by the e2-detector as well by extracting the value \textit{nVehSeen} for each second. Finally, the structure of $\boldsymbol{Y}$ is $[simulations \times timesteps \times lanes \times targets]$

\begin{figure}[h]
	\centering
	\includegraphics[width=0.6\textwidth]{deeplearning/model_topology.pdf}
	\caption[Topology of the deep learning model] {Topology of the deep learning model. } \label{bild.DL_model}
\end{figure}

After building $\boldsymbol{X}$ and $\boldsymbol{Y}$, the second-by-second data can be averaged over a certain time interval. In this thesis the time interval is chosen to be 10 seconds. By that, the size of the input data is reduced and the information density increased. $\boldsymbol{X}$ and $\boldsymbol{Y}$ can  now be used to train the model. The used model structure is shown in fig. \ref{bild.DL_model}.
The design matrix $\boldsymbol{X}$ is fed into the first GAT layer, which is supposed to learn spatial attention between the lanes. As a second input, the GAT layer receives the adjacency matrix $\boldsymbol{A}$. In fig. \ref{bild.DL_model} only one GAT layer for simplicity is shown. In the final approach two GAT layer are stacked together behind each other. The number of output features for both GAT layer is chosen to be 128, which was determined iteratively by trial and error. Generally, it is recommended to choose the number of features as a power of two to optimize storage usage. Since the GAT layer only take a matrix of the dimension $lanes \times features$ as an input to process the learning algorithm presented in \ref{sec:gat_layer}, wrapper-code is necessary, which feeds in the matrix for all time steps and for all simulations [$\forall simulations, \forall timesteps$]. The following Dense layer are fully connected layer which are presented in sec. \ref{sec:basics_NN}. The dense layer with the width of 128 are supposed to rearrange the learned features from the GAT layer in a way it is necessary for the following encoder-decoder structure. For this layer, the same wrapper-code is necessary, since fully connected layer only take a matrix as input. Following, the encoder takes the whole data for each simulation as an input, including the time steps. So for the encoder, the wrapper code is not necessary anymore, since the encoder handles the time steps sequentially (see sec. \ref{sec:enc-dec}). The inputs per time step are encoded to hidden states, which are used by the following attention decoder to decode the hidden states back into the output time sequence. The temporal attention mechanism is included in the decoder. Both, the encoder and attention decoder, have 128 units per hidden state. Generally, in this approach two different attention mechanism are used. In the GAT layer spatial attention is applied, while the decoder uses temporal attention to estimate the output sequence. 
Furthermore, $L^2$ regularization and dropout (see sec. \ref{sec:basics_NN}) after each GAT and dense layer are applied to avoid overfitting. During training, the loss function for the optimization algorithm is chosen as the mean squared error (MSE) between the prediction and the ground-truth data.

The entire procedure for training and testing the deep learning model starts with running several traffic simulations (e.g. 150) with all the same settings in SUMO and collecting for each of them the detector data. The single SUMO simulations are all different from each other although they have the same settings, since the traffic in SUMO is randomized. The used road network in SUMO is exactly the same then in sec. \ref{sec.liu_on_grid}. Based on the detector data the queue length estimation after chapter \ref{sec.liu_method} is executed for each simulation. Afterwards the collection of simulations are divided into training, validation as well as the test data and the $\boldsymbol{X}$ and $\boldsymbol{Y}$ matrices are build. During training, the gradient updates for the parameter are calculated based on the training data. The validation data are also used during training to calculate the validation loss and monitoring the success of the training regarding under- or overfitting. After the training is finished, the model is tested on the test data, which it has never seen before during training, to evaluate the performance. The results of this test data are presented in the following chapter. 

%-----------------------------------------------------------------------------
%Implementation:
%
%-> talk briefly about keras and tensorflow in python

%-> describe how a road network is modeled as a graph

%-> introduce model topology with arrangement of gat layer -> dense -> enc-dec

%-> describe time distributed wrapper

\section{Results} \label{sec.DL_results}

In this chapter the results of the introduced deep learning model are presented. The first part is about the practical usage of the mean average error (MAPE), and which problems result based on that. Furthermore, an alternative metric for evaluation, the \textit{mean average error} is introduced. Afterwards, the results from selected lanes are presented and the performance of the deep learning model is compared to the method of \cite{liu_real-time_2009}. In addition to that, the overall performance for the entire network for multiple simulations is presented. Afterwards, the difference of the estimation accuracy is discussed, in case the results from the method presented in \ref{sec.liu_method} (here in future called \textit{Liu-method}) is not an input feature for the deep learning model. Finally, the performance of the model is validated in case traffic light cycles or traffic arrival flow changes for the test data, compared to the training data. 

\begin{figure}[h]
	\centering
	\includegraphics[width=1\textwidth]{deeplearning/20181009_0_A_normal_run1_251/DL_result_queue_0-1to0-2_2.pdf}
	\caption[Example for not reliable MAPE] {
		Example for not reliable MAPE: \\
				\begin{tabular}{c|c|c|} 
					\cline{2-3}
					& \multicolumn{2}{c|}{\textbf{Queue estimation:}} \\
					& \textbf{DL model}     & \textbf{Liu-method}     \\ \hline
					\multicolumn{1}{|c|}{MAE {[}m{]}}           & 15                  & 67.1          \\ \hline
					\multicolumn{1}{|c|}{MAPE {[}\%{]}} & 190.9                  & 53.4           \\ \hline
				\end{tabular}
				} \label{bild.MAPE_problem}
\end{figure}

Before the final results are presented, it is important to emphasize the limitations of the MAPE for evaluation of the performance. Due to the fact that the MAPE measures the percentage error, the metric is not reliable anymore, when the ground-truth value goes close to zero, while the estimation has a larger value. This correlation is presented in fig. \ref{bild.MAPE_problem}, which is a real prediction from the trained DL model. The MAPE of the DL model (190.9\%) is worse than the MAPE of the Liu-method (53.4\%), although the DL model has a much better performance considering the impression of the graph in fig. \ref{bild.MAPE_problem}. The reason for that is located at the beginning of the time axis after 200 seconds. The ground-truth value is close to zero, while the estimated value of the DL model is at around 20 meters. Considering the the formula of the MAPE which is

\begin{equation}
MAPE = \frac{1}{m} \sum_{m} \bigm| \frac{Observation - Estimation}{Observation} \bigm| \times 100 \%,
\end{equation}

the phenomenon can be explained. When the observation is close to zero but the estimation is not, the result of the fraction becomes very high and does not represent the real performance of the estimation anymore. An alternative is the \textit{mean average error (MAE)}

\begin{equation}
	MAE = \frac{1}{m} \sum_{m} \bigm| Observation - Estimation \bigm|.
\end{equation}

The MAE does not have the problem of the exploding value in some cases, and is still interpretable, since it has the same dimension as the estimation (in this case meters or number of vehicle). Regarding fig. \ref{bild.MAPE_problem}, the MAE for the DL model is 15.0 meters while for the Liu-method 67.1 meters. In the following both metrics (MAPE and MAE) are presented, but in some cases the MAPE does not give reliable results.
In fig. \ref{bild.compare_simus} the results for another lane in the network are presented. Figure \ref{bild.compare_simus} (a) shows the estimated queue length from the DL model and Liu-method compared to the ground-truth data in the upper graph. The performance of the deep learning model is very accurate, it follows the ground-truth data very well. Especially the two maximums at 500 and 800 seconds are good estimated.
\begin{figure}[H]
	\centering
	\includegraphics[width=1\textwidth]{deeplearning/20181009_0_A_normal_run1_251/2_2to1_2.pdf}
	\caption[Comparison of results for the same lane from different test simulations] {Comparison of results for the same lane from different test simulations (DL model is the same). \\
		\begin{tabular}{c|c|c|c|}
			\cline{2-4}
			& \multicolumn{2}{c|}{\textbf{Queue estimation:}} & \textbf{nVehSeen:} \\
			& \textbf{DL model}     & \textbf{Liu-method}     & \textbf{DL model}  \\ \hline
			\multicolumn{1}{|c|}{MAE (a)}           & 10.5 m                & 43.2 m                  & 1.9 veh            \\ \hline
			\multicolumn{1}{|c|}{MAPE (a) {[}\%{]}} & 24.7                  & 59.3                    & 61124881.6         \\ \hline
			\multicolumn{1}{|c|}{MAE (b)}           & 13.2 m                & 31.8 m                  & 1.3 veh            \\ \hline
			\multicolumn{1}{|c|}{MAPE (b) {[}\%{]}} & 27.2                  & 50.4                    & 50774859.8         \\ \hline
		\end{tabular}} \label{bild.compare_simus}
\end{figure}
This is also represented by the MAPE (24.7\%) and MAE (10.5 m). The Liu-method underestimates, which is caused by the effect of stop-and-go traffic, discussed in sec. \ref{sec.liu_on_grid}, since the presented lane is a left-turn lane. 
The breakpoint C is detected too early, which results in continuous underestimation. The MAPE for the Liu-method is 59.3\% and the MAE 43.2 meter, which attest the better performance of the DL model. The Liu-method has the same issue for almost every left-turn lane in the road-network.
In the lower graph of (a) the estimation for the number of vehicles on the entire lane are shown. Due to the fact, that second-by-second data are used which are averaged to 10 second intervals, the graph seems to have a higher resolution than the upper graph for the queue length, where only one value per traffic light cycle is linear interpolated. Generally, the ground frequency depends on the traffic light phases. The neural network is able to detect the frequency and tries to estimate the peaks, which is not everywhere accurate. With a MAE of 1.9 vehicle (the MAPE is not reliable in this case), the performance is acceptable, but not perfect yet. 
In fig. \ref{bild.compare_simus} (b) results for exact the same lane in the same road network are shown. They are predicted by the same DL model, just for another test simulation. 
\begin{figure}[H]
	\centering
	\includegraphics[width=1\textwidth]{deeplearning/right_turn_example.pdf}
	\caption[Estimation results for a right-turn lane] {Estimation results for a right-turn lane. \\
		\begin{tabular}{c|c|c|c|}
			\cline{2-4}
			& \multicolumn{2}{c|}{\textbf{Queue estimation:}} & \textbf{nVehSeen:} \\
			& \textbf{DL model}     & \textbf{Liu-method}     & \textbf{DL model}  \\ \hline
			\multicolumn{1}{|c|}{MAE}           & 4.8 m                 & 19.8 m                  & 1.9 veh            \\ \hline
			\multicolumn{1}{|c|}{MAPE {[}\%{]}} & 16.5                  & 77.3                    & 33.9               \\ \hline
		\end{tabular}} \label{bild.right_turn_exmpl}
\end{figure}
This should emphasize two things: First, the simulation data generated by SUMO, which are used for training, validation and testing, are very different from each other. The goal is to have a high diversity in the data, so that the deep learning model is able to generalize knowledge and does not overfit.  
Second, although the DL model performs very well in (a), it has still a satisfying performance in (b) for a completely different ground-truth, which is also caused by the high diversity in the training data. The MAPE for the queue length in (b) is 27.2\% and the MAE is 13.2 meters. The Liu-method also suffers here from the stop-and-go traffic and underestimates.
In fig. \ref{bild.right_turn_exmpl} an example for a right-turn lane is shown. In this case, the DL model has satisfying performance with a MAPE of 16.5\% (MAE = 4.8 m), although it starts to "smooth out" after 1000 seconds. This effect could be caused by to many time steps that are taken into consideration for the decoding. The Liu-method is overestimating, since the lane is a right-turn lane where a lot of lane changes occur. Vehicles are changing after passing the advanced detector to other lanes, which cannot be handled by the Liu-method (discussed in sec. \ref{sec.liu_on_grid}). This is also shown by the MAPE (77.3\%) and MAE (19.8 m). For the estimation of nVehSeen, the curve is again smoothing and not very accurate. The MAPE (33.9\%) and MAE (1.9 veh) is also not completely satisfying. Also this could be caused by to many time steps, that are taken into consideration for the attention decoding. Especially for estimating the second target (nVehSeen), the optimal model configuration is not found yet. However, note that the approach has a lot of potential so far. This is also emphasized by considering the averaged MAPE and MAE for the entire road network (not only for a single lane, as presented above). In table \ref{tab.MAE_entire_net} the MAEs for several test simulations are presented. The MAPEs are not reliable sources, since at least one lane has a MAPE which has a very high (and not reliable) value.

\begin{table}[h]
	\centering
	\begin{tabular}{c|c|c|c}
		& \multicolumn{2}{c|}{\textbf{MAE queue length {[}m{]}}} & \textbf{MAE nVehSeen {[}veh{]}} \\ \hline
		\textbf{Simulation \#} & \textbf{DL model}         & \textbf{Liu-method}        & \textbf{DL model}               \\ \hline
		1                      & 9.1                       & 18.1                       & 1.4                             \\
		2                      & 9.5                       & 17.8                       & 1.5                             \\
		3                      & 9.0                       & 18.6                       & 1.6                             \\
		4                      & 8.9                       & 18.1                       & 1.4                             \\
		5                      & 9.4                       & 18.5                       & 1.5                             \\ \hline
		\textbf{Average:}      & 9.2                       & 18.2                       & 1.5                            
	\end{tabular}
	\caption[Estimation results (MAE) of an entire road-network] {Estimation results (MAE) of an entire road-network for five test simulations.} \label{tab.MAE_entire_net}
\end{table}

It turns out, that the performance of the deep learning model is very constant over different independent test simulations. In addition to that, the DL model has around twice better performance regarding the MAE than the Liu-method. For the number of vehicles on the entire lane (nVehSeen), the deep learning model has a MAPE around 1.5 vehicles, which is acceptable considering the number of vehicles that are on the entire lane, but there is no reference to other methods available.  

\subsection{Robustness for different Arrival Rates}

Although the performance, especially of the queue length estimation, is satisfying, it is important to note that the traffic parameter are the same for training and testing. For example the arrival rate of the traffic is the same, although the traffic routes for the single vehicles are randomized by SUMO. It would be interesting to analyze, how the DL model behaves when the input data have different arrival rates. This study is shown in fig. \ref{bild.03_period} for a selected left-turn lane.

\begin{figure}[h]
	\centering
	\includegraphics[width=1\textwidth]{deeplearning/03_period_test.pdf}
	\caption[Test of the DL model for different traffic arrival rate] {Test of the DL model for different traffic arrival rate.\\
\begin{tabular}{c|c|c|c|}
	\cline{2-4}
	& \multicolumn{2}{c|}{\textbf{Queue estimation:}} & \textbf{nVehSeen:} \\
	& \textbf{DL model}     & \textbf{Liu-method}     & \textbf{DL model}  \\ \hline
	\multicolumn{1}{|c|}{MAE}           & 75.6 m                & 149.6 m                 & 13.9 veh           \\ \hline
	\multicolumn{1}{|c|}{MAPE {[}\%{]}} & 45.6                  & 63.7                    & 148.5              \\ \hline
\end{tabular}
} \label{bild.03_period}
\end{figure}

The presented test data have a arrival rate of 3.33 veh/s while the DL model is only trained on data with 2.5 veh/s arrival rate. Regarding the estimation of the queue length, the DL model has some problems to estimate accurately the first maximum. But it still has with a MAE of 75.6 meters a better performance than the Liu-method with MAE = 149.6. The estimation of the nVehSeen is more critical. In the period of time between 650 and 1150 seconds, the estimated vehicles on the lane reach very high values. The DL model shows instable behavior. However, this behavior is expected, since it has never seen a nVehSeen of 20 during training before. So it has no knowledge about how to handle this situation. This is a common problem for any sort of statistical model which is used for prediction out of samples. The worse performance is also illustrated by the average MAEs for all lanes. The MAE for the DL model is 31.5 m, for the Liu-method 56.2 m and for the DL model estimating the nVehSeen the MAE is 5.9. 

\begin{figure}[H]
	\centering
	\includegraphics[width=1\textwidth]{deeplearning/03_period_test_new.pdf}
	\caption[Test of the DL model for traffic arrival rate of 0.3 sec/veh, when model is trained on multiple arrival rates] {Test of the DL model for traffic arrival rate of 0.3 sec/veh, when model is trained on multiple arrival rates.\\
		\begin{tabular}{c|c|c|c|}
			\cline{2-4}
			& \multicolumn{2}{c|}{\textbf{Queue estimation:}} & \textbf{nVehSeen:} \\
			& \textbf{DL model}     & \textbf{Liu-method}     & \textbf{DL model}  \\ \hline
			\multicolumn{1}{|c|}{MAE}           & 77.8 m                & 149.5 m                 & 4.4 veh           \\ \hline
			\multicolumn{1}{|c|}{MAPE {[}\%{]}} & 39.4                 & 63.7                    & 61.3              \\ \hline
		\end{tabular}\label{bild.03_period_new}
	} 
\end{figure}

The performance can be improved, if the model is not only trained with simulation data based on a specific arrival rate, but with a high diversity of arrival rates. If the deep learning model has a higher diversity in the training data, the generalization of knowledge is better. In fig. \ref{bild.03_period_new} the results are shown for the same DL model but trained with 180 simulations with a randomized arrival rate between 0.45 and 0.25 sec/veh for each simulation, rather than with 125 simulations of 0.4 sec/veh data as for fig. \ref{bild.03_period}. Since the data have a higher diversity, more simulations are necessary to allow similar performance. 

The performance of the queue length estimation in fig. \ref{bild.03_period_new} is not better compared to fig. \ref{bild.03_period} which has a MAE of (75.6 m). The reason is that 180 simulations are too less for training a model properly for all possible arrival rates. But it is still enough to stabilize the prediction for nVehSeen in the lower graph of fig. \ref{bild.03_period_new}. While in fig. \ref{bild.03_period} the nVehSeen becomes unstable and have a MAE of 13.9 veh, in fig. \ref{bild.03_period_new} the behavior is stable with a MAE of 4.4 veh. The model has already seen similar traffic situations during training and can handle the situation. The average MAEs for the entire network are compared in table \ref{tab.compare} for both different models.

\begin{table}[H] 
	\centering
	\begin{tabular}{|c|c|c|c|c|}
		\hline
		\multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Arrival rate\\  for training\\ {[}sec/veh{]}\end{tabular}}} & \multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Number of\\ training \\ simulations\end{tabular}}} & \multicolumn{2}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Queue estimation\\ MAE\\ (MAD)\end{tabular}}}                   & \textbf{\begin{tabular}[c]{@{}c@{}}nVehSeen\\ MAE\\ (MAD)\end{tabular}} \\ \cline{3-5} 
		&                                                                                                       & \textbf{DL model}                                          & \textbf{Liu-method}                                       & \textbf{DL model}                                                       \\ \hline
		\textbf{0.4}                                                                                                   & \textbf{125}                                                                                          & \begin{tabular}[c]{@{}c@{}}31.5 m \\ (30.2 m)\end{tabular} & \begin{tabular}[c]{@{}c@{}}56.2 m\\ (66.4 m)\end{tabular} & \begin{tabular}[c]{@{}c@{}}5.9 veh\\ (6.8 veh)\end{tabular}             \\ \hline
		\textbf{0.25 - 0.45}                                                                                           & \textbf{180}                                                                                          & \begin{tabular}[c]{@{}c@{}}24.7 m\\ (21.1 m)\end{tabular}  & \begin{tabular}[c]{@{}c@{}}56.2 m\\ (66.4 m)\end{tabular} & \begin{tabular}[c]{@{}c@{}}3.8 veh\\ (3.2 veh)\end{tabular}             \\ \hline
	\end{tabular}
	\caption[MAEs and MADs for the entire road network predicted by the same model which was trained on datasets with different arrival rates] {MAEs and MADs for the entire road network predicted by the same model which was trained on datasets with different arrival rates.} \label{tab.compare}
\end{table}

The MAE for the queue estimation is better for the deep learning model trained on multiple arrival rates compared to the model trained on only one arrival rate. Even better is the improvement for the estimated nVehSeen. As additional metric the \textit{mean absolute deviation (MAD)} is used, which is 
\begin{equation}
	MAD = \frac{1}{m} \sum_{i = 1}^{m} \mid MAE_i - \overline{MAE} \mid,
\end{equation}
where $m$ is the number of lanes and $\overline{MAE}$ is the average MAE for all lanes. The MAD is very high for both models due to the instable situations that occur for both. Still, the model trained on more arrival rates, has a lower MAD in all categories. 
 Furthermore, the DL model does not become instable in certain situations anymore. While for the old model on 16 of 120 lanes instability occurs, the improved model has 5 lanes where the nVehSeen becomes instable and overestimation occurs. The improved model has not the optimal performance yet, since a higher amount of simulations are necessary to gain reliability.
However, this demonstration should emphasize how important it is to train on many different relevant data as possible to have a maximum of generalized knowledge for every traffic case.

% show how dl model performs on changed traffic light cycles(optional if time left)
%train DL model with different traffic light cycles (optinal)

%-> verify that using the results from liu are gaining the accuracy of the estimation -> come to the conclusion, that it was worth it to do the preliminary work with liu

\subsection{Influence of Liu-Method as Input}

Finally, it is also important to investigate, if the usage of the Liu-method as an input feature is a benefit. Therefore, the exactly same model was trained twice. For the first dataset the results of the Liu-method were included (8 input features) which is in the following called \textit{with-Liu model}, for the second dataset the Liu-method was not included (7 input features) also called as \textit{no-Liu model}. 
In fig. \ref{bild.without_liu} the results of both training sessions are presented for the same lane. In fig. \ref{bild.without_liu} (a) the estimated queue length and nVehSeen for the model with Liu-method as input are presented, while in (b) the results for the model without Liu-method are shown. For the comparison of the estimated queue length, the no-Liu model with a MAE of 32.9 m seems to have almost the same performance as the with-Liu model with a MAE of 31.1 m. 
\begin{figure}[H]
	\centering
	\includegraphics[width=1\textwidth]{deeplearning/compare_w_wo_liu/figure_comparison.pdf}
	\caption[Comparison of results for the same lane if results of Liu-method are input feature or not] {Comparison of results for the same lane if results of Liu-method are input feature or not (DL model is the same). \\
		\begin{tabular}{c|c|c|c|}
			\cline{2-4}
			& \multicolumn{2}{c|}{\textbf{Queue estimation:}} & \textbf{nVehSeen:} \\
			& \textbf{DL model}     & \textbf{Liu-method}     & \textbf{DL model}  \\ \hline
			\multicolumn{1}{|c|}{MAE (a)}           & 31.1 m                & 121.7 m                  & 2.0 veh            \\ \hline
			\multicolumn{1}{|c|}{MAPE (a) {[}\%{]}} & 18.86                  & 68.2                    & 64.6         \\ \hline
			\multicolumn{1}{|c|}{MAE (b)}           & 32.9 m                & 121.8 m                  & 2.3 veh            \\ \hline
			\multicolumn{1}{|c|}{MAPE (b) {[}\%{]}} & 21.5                  & 68.2                    & 40.9         \\ \hline
		\end{tabular}} \label{bild.without_liu}
\end{figure}

The comparison between the estimated nVehSeen is more interesting: While the MAEs are also not significant different (2.0 veh for with-Liu and 2.3 veh for no-Liu) the difference between the graphs are higher. The nVehSeen in (a) (with-Liu) follow the ground truth curve quiet well with a slightly smoothing character. For the nVehSeen in (b) (no-Liu), the behavior of the estimation becomes sometimes instable with many drops, at some points the estimation is even below zero. It is suspected, that this unrealistic behavior is caused by overfitting of the training data. Not only on this particular lane, but also on 15 other lanes the estimated value drops 25 times in total below zero. This does not happen for the DL model in trained with the Liu-method as input. The average MAEs as well as the MADs of both models are compared in table \ref{tab.MAE_wo_liu}. 

\begin{table}[h]
	\centering
	\begin{tabular}{|c|c|c|c|c|}
		\hline
		\multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Usage\\ of\\ Liu-method\end{tabular}}} & \multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Number of\\ training \\ simulations\end{tabular}}} & \multicolumn{2}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Queue estimation\\ MAE\\ (MAD)\end{tabular}}}                 & \textbf{\begin{tabular}[c]{@{}c@{}}nVehSeen\\ MAE\\ (MAD)\end{tabular}} \\ \cline{3-5} 
		&                                                                                                       & \textbf{DL model}                                        & \textbf{Liu-method}                                       & \textbf{DL model}                                                       \\ \hline
		\textbf{w/ Liu}                                                                           & \textbf{125}                                                                                          & \begin{tabular}[c]{@{}c@{}}9.4 m \\ (5.3 m)\end{tabular} & \begin{tabular}[c]{@{}c@{}}18.1 m\\ (13.7 m)\end{tabular} & \begin{tabular}[c]{@{}c@{}}1.6 veh\\ (0.4 veh)\end{tabular}             \\ \hline
		\textbf{w/o Liu}                                                                          & \textbf{125}                                                                                          & \begin{tabular}[c]{@{}c@{}}9.0 m\\ (5.4 m)\end{tabular}  & \begin{tabular}[c]{@{}c@{}}18.1 m\\ (13.7 m)\end{tabular} & \begin{tabular}[c]{@{}c@{}}1.4 veh\\ (0.4 veh)\end{tabular}             \\ \hline
	\end{tabular}
	\caption[Estimation results (MAE) for model with and without Liu-method as input] {Estimation results (MAE) for model with and without Liu-method as input.} \label{tab.MAE_wo_liu}
\end{table}

Only considering the MAEs, the no-Liu model seems to be slightly better. Furthermore, there is no difference for the MADs between both models. However, this data do not represent the performance regarding the stability for the estimation of nVehSeen. The Liu-method used as input feature prevents the model from overfitting, which results in a more stable behavior of nVehSeen. In this case, prior knowledge about the traffic is used, to avoid overfitting and guide the model in the right direction. In this case, to add prior knowledge has similar effects than classic regularization techniques like dropout or $L^2$-Regularization. It would be also possible to avoid overfitting by using more training data, but in reality traffic data are rare and expensive. So it is beneficial for the learning process to have preprocessed data by the Liu-method as input, which saves some effort for data mining and computational cost for training. 

% --------------write stuff-----------------
%Results: (similar structure to presentation)
%
%-> present problem with MAPE and introduce MAE
%
%-> show results for different simulations for the same lane
%
%-> Present average MAPE and MAE for the entire road network
%
%-> try to improve performance by implementing attention horizon in attention decoder (not so important)
%
%-> test the model with different traffic light plans
%
%-> verify that using the results from liu are gaining the accuracy of the estimation -> come to the conclusion, that it was worth it to do the preliminary work with liu





==> abstract.tex <==
Due to urbanization and the increase of individual mobility, in most metropolitan areas around the world congestion and inefficient traffic management occur. The economical and ecological consequences of this phenomenon are harmful to the environment. Highly necessary intelligent traffic control systems, which are able to reduce congestion, rely on measurements of traffic situations in urban road networks and freeways. Unfortunately, the instrumentation for accurate traffic measurement is expensive and not widely implemented. This thesis addresses this problem, where relatively inexpensive and easy to install loop-detectors are used by a geometric deep learning algorithm, which uses loop-detector data in a spatial context of a road network, to estimate queue length in front of signalized intersections, which can be then used for following traffic control tasks. 
Therefore, in the first part of this work a conventional estimation method for queue length (which does not use machine learning techniques) based on second-by-second loop-detector data is implemented, which uses detected shockwaves in queues to estimate the length and point of time for the maximum queue. The method is later used as reference but also as additional input information for the geometric deep learning approach. In the second part the geometric deep learning algorithm is developed, which uses spatial correlations in the road network but also temporal correlations in detector data time sequences by new attention mechanisms, to overcome the limitations of conventional methods like excess traffic demand, lane changing and stop-and-go traffic. Therefore, it is necessary to abstract the topology of the road network in a graph. Both approaches are compared regarding their performance, reliability as well as limitations and validated by usage of the traffic simulation software SUMO (Simulation of Urban MObility). Finally, the results are discussed in the conclusions and further investigations are suggested.  


==> deeplearning/deeplearning.tex <==
\chapter{Queue Length Estimation with Geometric Deep Learning} \label{sec.geometric_deep_learning}

As demonstrated in section \ref{sec.liu_on_grid}, the estimation of the expansion model is not accurate for a realistic road network due to lane changes and stop and go traffic behavior. Therefore, in this work another approach with geometric deep learning will be examined. This approach is potential superior, since it is able to take spatial correlations into consideration due to graph attention mechanisms. Furthermore, it is expected the network is able to learn more complex relations like lane changing.
In the past few years a big progress was made in the field of \textit{neural sequence-to-sequence models}, especially applied to human language translation \cite{neubig_neural_2017}. The goal of this work is to apply these techniques on road networks for estimation and prediction of queue length and pressure. Generally, the model gets a time sequence containing of detector data as input and gives a time sequence of traffic queue length as output. 

In this chapter, the fundamentals which are important to implement geometric deep learning networks are presented. Furthermore, the implementation of the  deep learning network as well as the results are shown.

\section{Fundamentals of Geometric Deep Learning}

Deep learning approaches became very popular during the past decades, since they were successfully applied in many different fields to solve real-world problems. Especially deep learning had big achievements in the past in fields like human language translation, computer vision, robotics, search engines and many more. Deep learning is a name for a particular class of machine learning techniques. Many of the recent advancements in the field of artificial intelligence (AI) are based in deep learning techniques. In classic machine learning approaches the input data are manually preprocessed by humans, which is called feature engineering. These hand-designed features are the input for the artificial neural network (ANN) or any other sort of statistical model which predicts the output. The process of feature engineering can be a big effort and requires domain knowledge about the data from the application engineer. For more complex problems it is sometimes not even possible to create the features by hand, for example in the field of face recognition or speech-to-text applications where the inputs are pictures or time sequences. Deep learning has the approach to preprocess the input data by itself and abstract the features by using several layers of neural networks. Thereby, a lot of time and effort in the application process can be saved and more complex problems can be solved. A disadvantage is, that the higher amount of layers and parameters increases the computational effort \cite{goodfellow_deep_2016}. In this work, the input data are the detector data from the e1 (loop) detectors which are fed into the deep learning model. The hypothesis is that the deep learning model should abstract the relevant features by itself by using the knowledge of the spatial correlations within the road network (usage of graph attention layers). This makes this model to a \textit{geometric} deep learning model \cite{bronstein_geometric_2017}.

In this section the theoretical fundamentals about deep learning are presented, which are necessary to successfully implement geometric deep learning networks for queue length estimation. Section \ref{sec:basics_NN} starts with the basics and general introduction of feedforward neural networks. To extract spatial information from the inputs, graph attention layer is introduced in section \ref{sec:gat_layer}. Recurrent neural networks (RNNs), presented in section \ref{sec:RNN}, are used to store relevant information over multiple time steps and represent the main component for the  RNN encoder-decoder model introduced in section \ref{sec:enc-dec}.

\subsection{Basics of Feedforward Neural Networks} \label{sec:basics_NN}
 Feedforward neural networks are the most simple and fundamental kind of deep learning models.
 When it comes to solving real-world problems, neural networks have great characteristics like nonlinearity, parallelism, handling of uncertain and fuzzy information as well as the ability to generalize knowledge \cite{basheer_artificial_2000}. Generally, the aim of these models is to approximate a function $f^*$. The general formulation for a regression would be $ \boldsymbol{\hat{y}} = f(\boldsymbol{x}, \boldsymbol{W})$, where $\boldsymbol{x}$ is the input, $\boldsymbol{\hat{y}}$ the predicted output and $\boldsymbol{W}$ the weight matrix. During the training process, the optimization algorithm learns the parameters that $f$ approximates $f^*$ the best. These models are called feedforward neural networks, since the input is fed trough the network and results an output without a feedback loop. Once a feedback loop is implemented, the model is called recurrent neural network (see section \ref{sec:RNN}). 
 
 \subsubsection{Structure} \label{sec.structure}
 
 Inspired by biological neural networks, a complex artificial neural network consists of many simple elements (artificial neurons or nodes). The analogy between the biological neurons to the artificial neurons is presented in Fig. \ref{bild.neurons}.
 
 \begin{figure}[h]
 	\centering
 	\includegraphics[width=1\textwidth]{deeplearning/neuron_example.png}
 	\caption[Analogy between biologial and artificial neurons]{Analogy between biologial (left) and artificial neurons (right) \cite{basheer_artificial_2000}.} \label{bild.neurons}
 \end{figure}

At the artificial neuron, the inputs $x_1$ to $x_n$ are multiplied with the corresponding weights $w_1$ to $w_n$ and get summed-up (this process is called \textit{affine transformation}). Afterwards, the sum is an input for the activation function, which adds the nonlinearity to the model. In this particular case, the activation function is a step function, which only lets the value pass, if a threshold is reached. But there are also other functions possible (shown in Fig. \ref{bild.activation_functions}).
 \begin{figure}[h]
 	\centering
 	\includegraphics[width=1\textwidth]{deeplearning/activation_functions.png}
 	\caption[Activation functions for deep learning models]{Examples for activation functions: step-function (left), tanh function (middle) and the rectified linear unit (ReLU) function (right) \cite{neubig_neural_2017}.} \label{bild.activation_functions}
 \end{figure}
 According to \cite{goodfellow_deep_2016}, the most recommended default activation function for deep learning applications is the ReLU function, which is defined by $\sigma(z) = max\{0,z\}$. Due to its piecewise linear characteristic, it has good optimization properties for gradient-based optimization algorithms.   
 Generally, neural networks chain together many simple affine transformations and activation functions to represent more complex functions. Due to this simple structure, it is easier and more efficient to train.
 A very good example for explaining how deep neural networks in principle work, is solving the XOR problem. The visualization of the XOR problem is shown in Fig. \ref{bild.XOR_problem} on the left.
  \begin{figure}[h]
  	\centering
  	\includegraphics[width=1\textwidth]{deeplearning/XOR_problem.png}
  	\caption[The XOR problem in deep learning] {The XOR problem with the original $\boldsymbol{x}$ space of the XOR logic on the left and the transformed representation after the first hidden layer (learned $\boldsymbol{h}$ space) on the right \cite{goodfellow_deep_2016}.} \label{bild.XOR_problem}
  \end{figure}
  For the original $\boldsymbol{x}$ space of the XOR logic, it is not possible to classify between 1 and 0 just by dividing the space into two parts by a line, since there is no configuration of a line that would separate the zeros from the ones. According to the XOR logic, the value becomes only one if exactly one of the values $x_1$ or $x_2$ is one. So a basic linear model like
  
  \begin{equation}
  	y = \boldsymbol{w^T}\boldsymbol{x}+\boldsymbol{b}
  \end{equation} 
  
  with the weights $\boldsymbol{w}$ and the bias $\boldsymbol{b}$ is not able to model the XOR logic and divide the zeros from the ones. This problem can be solved by implementing a slightly more complicated structure by adding a \textit{hidden layer} and splitting the calculation in two steps.
  
  \begin{equation} \label{eq:hidden_layer}
  	\boldsymbol{h} = ReLu(\boldsymbol{W}_{xh}\boldsymbol{x}+\boldsymbol{b}_h)
  \end{equation}
  \begin{equation} \label{eq:output_layer}
  	y = \boldsymbol{w}_{hy}\boldsymbol{h}+b_y
  \end{equation}
Eq. \ref{eq:hidden_layer} represents the hidden layer which takes as inputs the vector $\boldsymbol{x}$ and outputs the vector $\boldsymbol{h}$. The transformed space $\boldsymbol{h}$ is shown in Fig. \ref{bild.XOR_problem} on the right. During the training process, the parameters $\boldsymbol{W}_{xh}$ and $\boldsymbol{b}_h$ are learned so that after the transformation it is possible to apply a linear model, which separates both patterns. This is done by the \textit{output layer} (eq. \ref{eq:output_layer}) to calculate the result $y$. In other words: The points in the $x$ space are transformed in the $h$ space by a matrix multiplication. In this new representation in the $h$ space, it is possible to separate the zeros from the ones by a line. The classification problem is solved by adding an additional hidden layer (eq. \ref{eq:hidden_layer}) to the linear model. The new structure of the model is shown in Fig. \ref{bild.XOR_structure}. 

  \begin{figure}[h]
  	\centering
  	\includegraphics[width=0.45\textwidth]{deeplearning/XOR_structure.png}
  	\caption[Structure of a model with one hidden layer] {Structure of the model to solve the XOR problem with one hidden layer. On the left side every node is drawn explicit and on the right side an simplified overview with the weights is given \cite{goodfellow_deep_2016}.} \label{bild.XOR_structure}
  \end{figure}

Generally, in a deep learning model are usually a lot more affine transformations and hidden layers so that more complex, multidimensional problems can be solved. But all this is based on very simple and easy computable affine transformations with following activation functions. So the first layer could be generally described as
\begin{equation} \label{eq:normal_NN}
	\boldsymbol{h}^{(1)} = \sigma^{(1)}(\boldsymbol{W}^{(1)}\boldsymbol{x}+\boldsymbol{b}^{(1)})
\end{equation}
with $\boldsymbol{x}$ as input and $\boldsymbol{W}^{(1)}$ as well as $\boldsymbol{b}^{(1)}$ as trainable parameters. The sum is input for the activation function $\sigma(\cdot)$. The second hidden layer is then given by
\begin{equation}
	\boldsymbol{h}^{(2)} = \sigma^{(2)}(\boldsymbol{W}^{(2)}\boldsymbol{h}^{(1)}+\boldsymbol{b}^{(2)})
\end{equation}
which takes now $\boldsymbol{h}^{(1)}$ as input. The activation functions $\sigma^{(i)}$ do not necessarily have to be the same. The next hidden layer takes $\boldsymbol{h}^{(2)}$ as input with its own weights and activation function and so on. The last layer of this series is called the \textit{output layer}. The \textit{depth} of the network is defined by number of layers that are chained together. The \textit{width} of the model is determined by the size of the outputs of the hidden layers $\boldsymbol{h}^{(i)}$.

How powerful it can be to transform the inputs into another representation is emphasized in Fig. \ref{bild.cartesian_polar}. 
  \begin{figure}[h]
  	\centering
  	\includegraphics[width=0.8\textwidth]{deeplearning/cartesian_polar_representation.png}
  	\caption[Comparison between patterns in cartesian and polar coordinates] {Comparison between patterns in cartesian and polar coordinates \cite{goodfellow_deep_2016}.} \label{bild.cartesian_polar}
  \end{figure}
Similar to the XOR-Problem, for this example it is also impossible to separate both patterns with a linear model when the representation is in cartesian coordinates. But it becomes possible once the points are transformed in polar coordinates by a hidden layer. Generally, the main task of layers in a neural network is to transform the inputs (features) into another coordinate-space, where it is possible to fulfill the original task which could be classification or linear regression. 

The optimal structure of a network with the depth, width and kind of activation functions can only be found in an experimental way, monitoring the errors for the training, test and validation set \cite{goodfellow_deep_2016}. To reach this goal, it is essential to understand the fundamentals how neural networks are trained and how optimization algorithms work. The following chapter provides a brief introduction in this field. 


\subsubsection{Training and Optimization}
%intoduce words like supervised learning, targets, freatures
Generally, neural networks are able to solve a variety of tasks, but they have to be specifically trained for this. These tasks can be for instance \textit{classification}, where the network determines the class the input data belongs to. An example would be an deep neural network which has animal pictures as input data and the task is to classify, whether in the picture is a cat, a dog or another animal. A different task would be \textit{regression}, where the output data are a  continuous graph. In this thesis, the presented neural network solves a regression problem, since it has to estimate the time sequence of the queue length based on time sequences of detector data as input. 
Another way to categorize learning algorithms is to differentiate between \textit{supervised} and \textit{unsupervised} learning. In case of machine/deep learning the input data are called \textit{features} $\boldsymbol{x}$ and the ground-truth output data are \textit{targets} or \textit{labels} $\boldsymbol{y}$. \textit{Unsupervised learning algorithms} though, use only the features for training without having corresponding targets. Usually the dataset has many features and the learning algorithm tries to learn correlations within the data. This can be used for tasks like denoising or clustering, where the dataset gets divided into several clusters containing data with similar properties .
For \textit{supervised learning algorithms} exist features $\boldsymbol{x}$ as well as corresponding targets $\boldsymbol{y}$. During training, the neural network model learns to predict $\boldsymbol{y}$ given the the input $\boldsymbol{x}$. This applies to this thesis, with the detector data as features $\boldsymbol{x}$ and the queue length as target $\boldsymbol{y}$. After training, the model should be able to predict an unknown $\boldsymbol{y}$ for a new $\boldsymbol{x}$. 
%mention briefly reinforcement learning, then introduce dataset, loss functions and then backprop
Another popular training method is \textit{reinforcement learning}, where the training model does not learn from a given dataset but from experience by interacting with an environment. But this is beyond the scope of this thesis \cite{goodfellow_deep_2016}. 

Summarized, in case of queue length estimation the approach is a regression problem which is solved by a supervised learning algorithm. For training of a deep neural network it is essential to have a large dataset, which contains of many examples with $n$ features ($\boldsymbol{x} \in \R^n$) and $m$ targets ($\boldsymbol{y} \in \R^m$). To describe the entire dataset with $k$ examples ($\boldsymbol{x}_1 ... \boldsymbol{x}_k$ and $\boldsymbol{y}_1 ... \boldsymbol{y}_k$), all of these examples are concatenated to a matrix $\boldsymbol{X} \in \R^{k \times n}$ (\textit{design matrix}) and $\boldsymbol{Y} \in \R^{k \times m}$.The symbol $k$ is called number of \textit{samples}. %now loss functions
During one training step in a supervised learning algorithm, the model gets one example $\boldsymbol{x}$ and predicts the output $\boldsymbol{\hat{y}}$. After the prediction, $\boldsymbol{\hat{y}}$ is compared to the provided ground-truth $\boldsymbol{y}$. This is usually made by \textit{loss functions}. The most common function for regression problems is the \textit{mean squared error} which is for $n$ features

\begin{equation}
	MSE = \frac{1}{n} \sum_{i=1}^{n} (\boldsymbol{\hat{y}}_i^2 - \boldsymbol{y}_i^2).
\end{equation}

If in one training step more than one example is used, the average of every single MSE is calculated. The loss determines how good the prediction is regarding the target. The goal of the training algorithm is to adjust the weights of the neural network, so that the loss gets reduced and the prediction converges to the target. Generally, to minimize the loss is a classic numerical optimization problem, which can be solved by well known numerical optimization algorithms. The most common optimization algorithms are \textit{gradient-based} algorithms. They use the derivative of the function (in this case the deep learning model represents the function) to get information about how to adjust $\boldsymbol{x}$ (or hidden states $\boldsymbol{h}$) in order to minimize the MSE between $\boldsymbol{\hat{y}}$ and $\boldsymbol{y}$. The simplest method is the \textit{gradient descent}, where $\boldsymbol{x}$ (or $\boldsymbol{h}$) is moved in the direction of the opposite sign of the derivative \cite{goodfellow_deep_2016}. 
For a successful optimization it is essential to determine the derivatives in the neural network model. 
% explain principle of back-propagation and why it is necessary. How is it implemented in computer?
In the previous subsection \ref{sec.structure} the fundamental structure is presented. It is shown, how the input $\boldsymbol{x}$ propagates trough the network and is computed, so that the output $\boldsymbol{\hat{y}}$ results. This process is called \textit{forward propagation}. During training, the forward propagation of the training data $\boldsymbol{x}$ results in the estimated output $\boldsymbol{\hat{y}}$. For convenience, the simple model from eq. \ref{eq:hidden_layer} and \ref{eq:output_layer} are shown again extended with the loss $l$ and modeled the ReLu function as a single step:

\begin{equation}
	  \begin{split} \label{eq:simple_model1}
	  \boldsymbol{h^{\prime}} &= \boldsymbol{W}_{xh}\boldsymbol{x}+\boldsymbol{b}_h \\
	  \boldsymbol{h} &= ReLu(\boldsymbol{h^{\prime}}) \\
	  \hat{y} &= \boldsymbol{w}_{hy}\boldsymbol{h}+b_y \\
	  l &= (\hat{y} - y)^2\\
	  \end{split}
\end{equation}

The derivatives of this model can be calculated by a method called \textit{back propagation}. With the chain rule the derivatives can be calculated for every set of weights. 

\begin{equation}
\begin{split} \label{eq:derivatives}
	\frac{dl}{db_y} &= \frac{dl}{d\hat{y}}\frac{d\hat{y}}{db_y} \\	
	\frac{dl}{d\boldsymbol{w}_{hy}} &= \frac{dl}{d\hat{y}}\frac{d\hat{y}}{d\boldsymbol{w}_{hy}} \\	
	\frac{dl}{d\boldsymbol{b}_h} &= \frac{dl}{d\hat{y}}\frac{d\hat{y}}{d\boldsymbol{h}}\frac{d\boldsymbol{h}}{d\boldsymbol{h^{\prime}}}\frac{d\boldsymbol{h^{\prime}}}{d\boldsymbol{b}_h} \\	
	\frac{dl}{d\boldsymbol{W}_{xh}} &= \frac{dl}{d\hat{y}}\frac{d\hat{y}}{d\boldsymbol{h}}\frac{d\boldsymbol{h}}{d\boldsymbol{h^{\prime}}}\frac{d\boldsymbol{h^{\prime}}}{d\boldsymbol{W}_{xh}} \\	
\end{split}
\end{equation}

In eq. \ref{eq:derivatives} the derivatives for all the weights regarding the loss function are presented. The chain rule allows to calculate the derivatives for every single step in the back propagation and multiply the results to get the derivatives for every single weight.
The derivations can become very complicated for larger networks so that it is impossible to calculate them by hand. Fortunately, it is possible to let the computer calculate the derivatives by using \textit{automatic differentiation (autodiff)}, where the feedforward propagation is modeled in many single steps (e.g addition, multiplication, square, ...) and the single derivatives are computed. So it is possible to create large networks and provide for every single neuron the forward function and the backward derivative computation \cite{neubig_neural_2017}.  

Once the forward propagation and the derivatives can be provided, the numerical gradient-based optimization algorithm is able to adjust the weights and minimize the loss. 
The fundamental form of the gradient descent algorithm is 
\begin{equation}
	\boldsymbol{x^{\prime}} = \boldsymbol{x} - \epsilon\boldsymbol{\nabla}_{\boldsymbol{x}}f(\boldsymbol{x})
\end{equation}

where $\boldsymbol{x^{\prime}}$ is the new approximation for the minimum, $\epsilon$ is the \textit{learning rate} and $\boldsymbol{\nabla}_{\boldsymbol{x}}f(\boldsymbol{x})$ is the gradient of $f$ which contains the partial derivatives. The learning rate is a fundamental \textit{hyperparameter}. Hyperparameters are parameters which control the learning algorithm. Further down in this section a few more will be introduced. 
The learning rate is important, since it has high influence on the training algorithm. If $\epsilon$ is too low, it takes a lot of training steps to reach the global minimum, which is highly inefficient. Furthermore it is possible, that the algorithm only finds a local minimum but not a global. Multidimensional optimization problems often have more than one minimum. This is visualized for a simple one dimensional case in fig. \ref{bild.multiple_minima}.

\begin{figure}[h]
  	\centering
  	\includegraphics[width=0.8\textwidth]{deeplearning/multiple_minima_plot.png}
  	\caption[Multiple minima in an optimization problem] {Multiple minima in an optimization problem \cite{goodfellow_deep_2016}.} \label{bild.multiple_minima}
\end{figure}

 If the learning rate is too high, it is possible that the algorithm cannot find a acceptable minimum either, since the algorithm "jumps" over the minimum. 
 The probably most common and used optimization algorithm for machine and deep learning is \textit{stochastic gradient descent} (SGD), which is a modification of the gradient descent method. Instead of computing the gradient based on only one example, SGD uses a minibatch of multiple examples to compute the average gradient. This results in a better generalization of the knowledge, since more parallel information are taken into consideration. Addressing the problem of the right choice of the learning rate, algorithms with adaptive learning rates have been developed. The most important in the field of deep learning are \textit{AdaGrad}, \textit{RMSProp} and \textit{Adam}. To present the algorithms in detail is beyond the scope of this thesis. \cite{goodfellow_deep_2016} gives a good overview of this topic. 
%show graphic with nice optimization algorithm and stepsize and so on... (implement maybe later, but no musthave!)

One of the main challenges when it comes to train neural networks is the phenomenon of \textit{underfitting} and \textit{overfitting}. Before training the model, the entire dataset is split into the \textit{training data} and \textit{test data}. The model is trained with the training data and afterwards the \textit{training loss} can be calculated. Furthermore, the model is tested on the test data it has never seen before during training. For the test session, the tests loss could be calculated as well. The ability of a model to make good predictions on data it has never observed before is called \textit{generalization}. The losses for training and testing over the \textit{model capacity} is shown in fig. \ref{bild.Loss_over_capacity} for a specific problem, which is not trivial but also not too complex. 
\begin{figure}[h]
	\centering
	\includegraphics[width=1\textwidth]{deeplearning/Loss_over_capacity.png}
	\caption[Underfitting and overfitting regarding model capacity] {Underfitting and overfitting regarding model capacity \cite{goodfellow_deep_2016}.} \label{bild.Loss_over_capacity}
\end{figure}
Simplified, the model capacity describes the complexity of the model regarding the number of hidden layers, the width and other structural properties. Models with a low capacity are not able to solve more complex problems. This leads to underfitting, where the training loss as well as the test loss is very high. The model cannot generalize knowledge, since it cannot even learn the information provided by the training data. Overfitting occurs if the model capacity is too high for the complexity of the given problem. The model has enough parameter to learn the whole training set, which results in a low training loss. The test loss is high though, because the model memorizes learned properties from the individual test data, which are not relevant for solving the problem. 
\begin{figure}[H]
	\centering
	\includegraphics[width=0.6\textwidth]{deeplearning/graph_under_overfitting.png}
	\caption[Visualization of the impact of underfitting and overfitting] {Visualization of the impact of underfitting and overfitting \cite{basheer_artificial_2000}.} \label{bild.under_overfitting}
\end{figure}
In this case, the model cannot generalize the knowledge either. This phenomenon is presented in detail in fig. \ref{bild.under_overfitting}.
For easier understanding of the figure, the model can be interpreted as a polynomial function. If the model complexity is too low (in this case polynomial of order one), the curve cannot fit the training points and also fails for an accurate prediction of the test points (both training and test loss are high). This is the classic case of underfitting. When the model complexity is increased to a polynomial function of second order, it fits quiet well for the training data but still has a rest loss, which is not zero. It also has a low loss for the test points, which is in this case the optimal solution. If the order of the polynomial increases even more (e.g order nine), the curve fits trough all the training points and the training loss is zero. But when it comes to predict the test points, the graph does not fit anymore and the test loss is very high. Then the model is overfitted. 

It is crucial to find the optimal model capacity to avoid underfitting or overfitting. The necessary complexity of the model highly depends on the individual problem to be solved. So there is no other way than using the trial-and-error method and maybe having experience from other applications. In addition to that, it is also possible (and recommended) to use regularization techniques during the training. Regularization has the aim to avoid overfitting and reduce the test loss on cost of an increasing train loss. In this section, only two (for this thesis relevant) regularization methods are briefly introduced. The first is \textit{parameter norm penalties}, in particular the $L^2$ \textit{parameter regularization}. 
\begin{figure}[H]
	\centering
	\includegraphics[width=0.6\textwidth]{deeplearning/L2_regularization.png}
	\caption[Visulaization of the $L^2$ regularization] {Visualization of the $L^2$ regularization \cite{goodfellow_deep_2016}. The point $\boldsymbol{w}^*$ represents the optimal parameter $w_1$ and $w_2$ to fit the training data. The dotted circles represent the increasing value of the penalty term with increasing distance to the origin. The optimum can be found in the point $\tilde{\boldsymbol{w}}$}. \label{bild.L2_regularization}
\end{figure}
Generally, for parameter regularization a penalty term is added to the loss functions which contains the weights $\boldsymbol{W}$ of each hidden layer. In case of the $L^2$ regularization the penalty term is $\Omega = \frac{1}{2} \lVert \boldsymbol{W} \rVert_2^2$. This additional term reduces high weights and overfitting to a particular training set. This method is also called \textit{weight decay}. 
In fig. \ref{bild.L2_regularization} the influence of the parameter regularization is presented.
Shown are the weights $\boldsymbol{w}^*$ which represents the parameter which would optimal fit the training dataset. The ellipses around this point visualize the increasing loss function without the penalty term for the parameter $w_1$ and $w_2$. The dotted circles represent the increasing value of the penalty term based on $w_1$ and $w_2$. The optimum between both the ellipses and dotted circles can be found in the point $\tilde{\boldsymbol{w}}$. In this way the $L^2$ regularization avoids the overfitting of the parameters to the point $\boldsymbol{w}^*$.
Another common regularization technique is \textit{dropout}. When dropout is applied during training, some weights are randomly set to zero. This creates a subnetwork of the original neural network which is then trained. In the next training step other weights are randomly chosen to be set to zero. This technique reduces on the one hand the capacity of the model which results in a need for higher number of nodes which requires more computational effort. On the other hand it reduces overfitting, since the structure of the neural network changes slightly in every training step. 

%\begin{equation}
%	\forall \; simulation, \forall \; timestep < t
%\end{equation}

The here briefly presented methods are fundamental for creating and training a deep learning model. However, deep learning is a large topic with many different applications and methods. A very good overview and introduction gives \cite{goodfellow_deep_2016}. In this thesis the focus in the following sections is on attention mechanisms and sequence to sequence problems in deep learning. Since in this approach the model uses data which have spatial correlations (lanes are connected to each other), it is beneficial to use attention mechanisms to let the model focus on relevant information.


\subsection{Graph Attention Networks} \label{sec:gat_layer}
The here presented \textit{graph attention networks} are designed to perform on geometric graphs which consist of \textit{nodes} and \textit{edges}. Each node is connected with other nodes by edges. Examples for graphs are social networks, road networks or 3D meshes. The structure does not necessarily have to be a grid-like structure. 
For solving tasks where it is possible to model correlations between data in a graph structure, it is often helpful to consider not only a single node, but its neighboring nodes. If the algorithm uses deep learning attention mechanisms for that, this process is called \textit{graph attention}. In this section a new method for learning attention for a graph, based on \cite{velickovic_graph_2017}, is presented. Described is a single \textit{graph attentional layer (GAT)}, which can be used to build larger graph attention networks. The input for this layer is a matrix which consists of every node of the graph including its features $\boldsymbol{h}_i$

\begin{equation}
	\boldsymbol{H} = \{\boldsymbol{h}_1,\boldsymbol{h}_2,...,\boldsymbol{h}_N\},\boldsymbol{h}_i \in \R^F, \boldsymbol{H} \in \R^{N \times F}.
\end{equation}

where $N$ is the number of nodes and $F$ is the number of features. The second input for the GAT layer is the information about the connections of the nodes in the graph. It is represented by the \textit{adjacency matrix}

\begin{equation}
	\boldsymbol{A} \in \{0, 1\}^{N \times N}.
\end{equation}

$\boldsymbol{A}$ is a binary matrix with the size number of nodes by number of nodes. If a node has a connection to another node, the value at this specific place in the matrix is one, otherwise it is zero. Before computing the output features for every node, it is necessary to compute \textit{attention coefficients} $e_{ij}$ for every node $i$ and its corresponding neighbors $j$ in the \textit{neighborhood} $\mathcal{N}_i$. The neighborhood $\forall \boldsymbol{h}_i: \mathcal{N}_i$ can be extracted by using the adjacency matrix. The single attention coefficients are calculated by

\begin{equation}
	e_{ij} = \sigma (\boldsymbol{a}^T [\boldsymbol{Wh}_i \lVert \boldsymbol{Wh}_j])
\end{equation}

with the \textit{weight matrix} $\boldsymbol{W} \in \R^{F^{\prime} \times F}$, where $F^{\prime}$ is the number of the new output features, and a \textit{weight vector} $\boldsymbol{a} \in \R^{2F^{\prime}}$. Furthermore, the $\lVert$ symbol represents the concatenation of the results of both matrix multiplications $\boldsymbol{Wh}_i$ for the node itself and $\boldsymbol{Wh}_j$ for the neighboring node. Afterwards the attention coefficients are normalized by a \textit{softmax} function, which allows a comparison between the coefficients:

\begin{equation}
\alpha_{ij} = \frac{exp(e_{ij})}{\sum_{k \in \mathcal{N}_i} exp(e_{ik})}.
\end{equation}

After the normalization, it is possible to calculate the new hidden state of the node $i$ by executing one learnable linear transformation and weighting it with the normalized attention coefficient for every node in the neighborhood of the node (including the node itself):

\begin{equation}
\boldsymbol{h}^{\prime}_i = \sigma \Big( \sum_{j \in \mathcal{N}_i} \alpha_{ij} \boldsymbol{Wh}_j  \Big) ; \quad \boldsymbol{h}^{\prime}_i \in \R^{F^{\prime}}
\end{equation}

Generally, the normalized attention coefficient $\alpha_{ij}$ decides, how much the former features from node $j$ contributes to the new hidden state $\boldsymbol{h}_i^{\prime}$ of node $i$. 

\begin{figure}[h]
	\centering
	\includegraphics[width=0.65\textwidth]{deeplearning/pic_attn_heads.pdf}
	\caption[Visualization of graph attention mechanism with tree attention heads] {Visualization of graph attention mechanism with three attention heads \cite{velickovic_graph_2017}.} \label{bild.annt_mechanism}
\end{figure}

Furthermore, \cite{velickovic_graph_2017} notes that it can be helpful to execute the calculation of attention coefficients and new hidden states multiple times independently from each other. By that the attention learning process can be more stabilized. This is then called "\textit{multi-head attention}" \cite{velickovic_graph_2017}. After the execution of $K$ different independent estimations with the attention mechanism, one way to process the results is to concatenate them:

%formula concatenating
\begin{equation}
\boldsymbol{h}^{\prime}_i = \overset{K}{\underset {k=1}{\lVert}} \;
\sigma \Big( \sum_{j \in \mathcal{N}_i} \alpha_{ij}^k \boldsymbol{W}^k\boldsymbol{h}_j  \Big); \quad \boldsymbol{h}^{\prime}_i \in \R^{F^{\prime}}
\end{equation}

where $k$ stands for each single attention head. Also each independent attention mechanism has its own attention coefficients $\alpha_{ij}^k$ and weight matrix $\boldsymbol{W}^k$. When using concatenation of the single results, the final number of features will be $KF^{\prime}$ instead of $F^{\prime}$. Another option to process the single results from each attention head is to average over $K$

%formula averaging
\begin{equation}
\boldsymbol{h}^{\prime}_i = 
\sigma \Big( \frac{1}{K} \sum_{k=1}^{K} \sum_{j \in \mathcal{N}_i} \alpha_{ij}^k \boldsymbol{W}^k\boldsymbol{h}_j  \Big); \quad \boldsymbol{h}^{\prime}_i \in \R^{KF^{\prime}}
\end{equation}

where all the single results are summed-up and divided by the number of attention heads. In this case, the number of output features per node is $F^{\prime}$.
In fig. \ref{bild.annt_mechanism} a visualization of the attention mechanism with three attention heads is presented. In this picture $\boldsymbol{h}_1$ are the old features of node one, while $\boldsymbol{h}_2$ to $\boldsymbol{h}_6$ are the neighboring nodes. Each of them contributes, scaled by the attention coefficients $\boldsymbol{\alpha}_{1j}$, to the new hidden state $\boldsymbol{h}_1^{\prime}$. The different parallel attention heads are visualized by the colored arrows. 
Finally, the output of the GAT layer is a matrix which contains all the features for each node in the graph:

\begin{equation}
	\boldsymbol{H}^{\prime} = \{\boldsymbol{h}_1^{\prime},\boldsymbol{h}_2^{\prime},...,\boldsymbol{h}_N^{\prime}\},\boldsymbol{h}_i^{\prime} \in \R^{F^{\prime}}, \boldsymbol{H}^{\prime} \in \R^{N \times F^{\prime}}
\end{equation}

Based on the presented single GAT layer, more complex networks can be build by using more than one graph attention layer in a network. 
%Specifically for solving the problem of queue length estimation, the GAT layer can help to take traffic data from other connected lanes into consideration. This can help to make the estimation more accurate. 

\subsection{Recurrent Neural Networks (RNN)} \label{sec:RNN}

All networks that have been presented in the previous chapters were feedforward neural networks. The information from the input propagates through the network and generates an output. Every new sample as input for the deep learning model is independent from the previous or following one. Also the order of the input-examples is mostly not very relevant. 
This becomes different when the input changes to sequences. 

Sequences can be for instance sentences (sequence of words) and the task is to translate this sequence into another language. So the input is a sequence and the output is a sequence as well. The models which are used to solve this task are called \textit{sequence-to-sequence (seq2seq) models} \cite{neubig_neural_2017}. Another example are time sequences, like in the approach which is made in this thesis. The input is a time sequence of loop-detector data and the output is the queue length in form of a time sequence as well. In the case of sequences, the single steps of the sequence are not independent from each other anymore but correlated to each other. For example in the sentence "\textit{He} loves \textit{his} red bike", the third word "his" is correlated to the first word "He". It matches regarding the gender. So a deep learning model structure is necessary which reads in every single step, but does not treat them independently, but as a sequence. Therefore, \textit{recurrent neural networks (RNN)} were developed, which are able to process sequential data. These family of networks have an internal feedback loop, where the calculated hidden state $\boldsymbol{h}_{i-1}$ from the previous step is fed back as an input of the model to calculate the new hidden state $\boldsymbol{h}_i$ for the current step. This allows the network to take also information from previous steps into consideration. In fig. \ref{bild.RNN_unfold} the general topology of a RNN is presented. 

\begin{figure}[h]
	\centering
	\includegraphics[width=1\textwidth]{deeplearning/RNN_unrolled.pdf}
	\caption[Unfold RNN] {Circuit diagram of the RNN (right) and its unfolded visualization (left) after  \cite{goodfellow_deep_2016}.} \label{bild.RNN_unfold}
\end{figure}

On the left site, the circuit diagram of the RNN is presented, where for the time step $i$ the RNN has as input $\boldsymbol{x}_i$ as well as the previous hidden state $\boldsymbol{h}_{i-1}$. In this case the RNN has no other output than its hidden state, but it is also possible to add another layer to compute an output. This is presented later in section \ref{sec:enc-dec}. On the right side, the unfold visualization with every time step is presented. It is important to note, that the recurrent neural network is for every time step the same with the same weights \cite{goodfellow_deep_2016}. 
The general equation to calculate the new hidden state is

\begin{equation}
	\boldsymbol{h}_i = \sigma(\boldsymbol{W}_{xh} \boldsymbol{x}_i + \boldsymbol{W}_{hh}\boldsymbol{h}_{i-1}+\boldsymbol{b}_h).
\end{equation}

The only difference between a normal feedforward neural network (see eq. \ref{eq:normal_NN}) and a recurrent neural network is the term $\boldsymbol{W}_{hh}\boldsymbol{h}_{i-1}$. The first hidden state $\boldsymbol{h}_0$ has to be initialized, which is usually a vector of zeros. The reason why recurrent neural networks can deal with long distance dependencies is, that all relevant information of previous time steps are stored in the hidden state $\boldsymbol{h}_{i-1}$ \cite{neubig_neural_2017}. 

The presented structure above is very simple and a straight forward development from a feedforward neural network. However, it has limitations due to the \textit{vanishing gradient} or \textit{exploding gradient} problem. The procedure to train a RNN is the same than for a normal neural network, which includes the forward propagation based on the input and following the back propagation using the gradients to optimize the weights. But in case of a RNN, the back propagation includes all previous time steps of the input sequence. If $\frac{d\boldsymbol{h}_{i-1}}{d\boldsymbol{h}_i}$ is not exactly one, the gradient between the hidden state at time step $i$ and the loss function $\frac{dl}{d\boldsymbol{h}_i}$ becomes either very small or very large. That means for a very long sequence, it is possible that the gradient at the beginning of the sequence is too small to have an effect to update the weights. 
The most popular solution for solving the vanishing and exploding gradient problem was introduced by \cite{hochreiter_long_1997} in 1997 and called \textit{long-short-term-memory (LSTM)}. It uses parallel to the hidden state $\boldsymbol{h}_i$ a \textit{memory cell} $\boldsymbol{c}$ which long and short term dependencies can be stored. Since $\frac{d\boldsymbol{c}_{i-1}}{d\boldsymbol{c}_i}$ is exactly one, no vanishing or exploding of the gradients occur. The LSTM can control which knowledge to keep in the memory cell and which knowledge to delete by using so called \textit{gates}. It uses \textit{input} and \textit{output} \textit{gates}, which both consist of an affine transformation with a following activation function. So the LSTM can learn, how to manage the information and which knowledge to keep over time and which not. LSTM had great success in solving seq2seq problems during the past years \cite{neubig_neural_2017}. 
However, in this thesis another variation of a recurrent neural network, which is called \textit{gated recurrent unit (GRU)}, will be used. It was first presented in \cite{cho_learning_2014} in 2014 and can be described as a simplification of an LSTM. It has no memory cell $\boldsymbol{c}$ but only uses the hidden state $\boldsymbol{h}$ for storing long term dependencies. It also has only two gates which are the \textit{update gate} $\boldsymbol{z}$ and the \textit{reset gate} $\boldsymbol{r}$. Although it is a simplification, the performance regarding sequence processing can be similar to an LSTM \cite{chung_empirical_2014}. The main structure is presented in fig. \ref{bild.GRU}. 

\begin{figure}[h]
	\centering
	\includegraphics[width=1\textwidth]{deeplearning/GRU.pdf}
	\caption[Visualization of a gated recurrent unit (GRU)] {Visualization of a gated recurrent unit (GRU) with the reset gate $\boldsymbol{r}$, update gate $\boldsymbol{z}$ and proposal hidden state $\boldsymbol{\tilde{h}}$ after  \cite{cho_learning_2014}. } \label{bild.GRU}
\end{figure}

The hidden state from the previous time step $\boldsymbol{h}_{i-1}$ as well as the current time step from the input sequence $\boldsymbol{x}_i$ are fed into the GRU. The first step is to calculate the proposed new hidden state

% calculate new proposal state
\begin{equation}
\boldsymbol{\tilde{h}}_i = tanh(\boldsymbol{Wx}_i+\boldsymbol{U}[\boldsymbol{r}_i \circ \boldsymbol{h}_{i-1}]+\boldsymbol{b})
\end{equation}

by using $\boldsymbol{h}_{t-1}$ and $\boldsymbol{x}_i$. The input $\boldsymbol{x}_i$ is multiplied with the weight matrix $\boldsymbol{W}$. Furthermore, $\boldsymbol{U}$ weights the element-wise multiplication ($\circ$) between the reset gate $\boldsymbol{r}_i$ and $\boldsymbol{h}_{i-1}$. The reset gate controls, which information of the previous hidden state contributes to the proposal state. The reset gate can be calculated as

%reset gate r_i
\begin{equation}
\boldsymbol{r}_i = \sigma (\boldsymbol{W}_r \boldsymbol{x}_i + \boldsymbol{U}_r \boldsymbol{h}_{i-1}+ \boldsymbol{b}_r).
\end{equation}

The calculation of the new hidden state is

%update new hidden state
\begin{equation}
\boldsymbol{h}_i = (1-\boldsymbol{z}_i)\circ \boldsymbol{h}_{i-1}+\boldsymbol{z}_i \circ \boldsymbol{\tilde{h}}_i; \quad \boldsymbol{h}_0 = \boldsymbol{0}
\end{equation}

where the update gate determines the ratio between the contribution of the previous and the proposal hidden state. The update gate can be calculated as

% update gate z_i
\begin{equation}
\boldsymbol{z}_i = \sigma (\boldsymbol{W}_z \boldsymbol{x}_i + \boldsymbol{U}_z \boldsymbol{h}_{i-1} + \boldsymbol{b}_z)
\end{equation}

with the weight matrices $\boldsymbol{W}_z$ and $\boldsymbol{U}_z$. Due to this structure, the GRU is able to solve tasks with long time dependencies in a sequence and still having a quiet simple model complexity \cite{cho_learning_2014}\cite{bahdanau_neural_2014}. Gated recurrent units are the main component for the processing sequences with an encoder-decoder structure, which is presented in the following section.
 

\subsection{RNN Encoder-Decoder} \label{sec:enc-dec}

The best approach to solve sequence-to-sequence models, is to use an \textit{RNN Encoder-Decoder} structure. Generally, two recurrent neural networks are sequentially used. The first RNN is the encoder, which gets a sequence as input and encodes it into hidden states. The decoder maps the information in the hidden states back into the output sequence. This algorithm is presented in \cite{cho_learning_2014}. In this thesis both RNN, the encoder and decoder, are GRU. In addition to that, in this thesis an \textit{attention decoder} based on \cite{bahdanau_neural_2014} is used. The attention mechanism is supposed to learn temporal attention within the time sequence. The main structure of the Encoder-Attention Decoder is presented in fig. \ref{bild.RNN_enc_dec}.

\begin{figure}[h]
	\centering
	\includegraphics[width=1\textwidth]{deeplearning/Encoder_Decoder_variant.pdf}
	\caption[Main structure of the RNN Encoder-Attention Decoder] {Main structure of the RNN Encoder-Attention Decoder in unfolded visualization. The encoder is presented in green, the attention mechanism in red and the decoder in blue \cite{cho_learning_2014}. } \label{bild.RNN_enc_dec}
\end{figure}

The encoder takes the input sequence $\boldsymbol{x}_1...\boldsymbol{x}_T$ and encodes it into hidden states for every time step. This process is equal to the GRU presented in the previous section \ref{sec:RNN}. The hidden state $\boldsymbol{h}_i$ has information about the current and all the previous inputs. The initial state $\boldsymbol{h}_0$ is chosen to a vector of zeros. 
The attention mechanism takes all the hidden states from the previous and current time step $\boldsymbol{h}_1 ... \boldsymbol{h}_i$ as well as the previous hidden state from the decoder $\boldsymbol{s}_{i-1}$ and calculates the \textit{context vector} $\boldsymbol{c}_i$ for every time step as

%context vector
\begin{equation}
	\boldsymbol{c}_i = \sum_{j=1}^{i}\alpha_{ij}\boldsymbol{h}_j
\end{equation}

with the normalized attention coefficients $\alpha_{ij}$ for every previous and the current time step $1...i$ regarding the current time step $i$. In the convex combination $\alpha_{ij}$ decides, how much the hidden state from each time step contributes to the calculation of the new output by the decoder. The original source \cite{bahdanau_neural_2014} takes all hidden states from all time steps (past and future) into consideration, since the original application is in the field of language translation, where the full sequence is already known in advance. In this case, the attention mechanism takes only the time steps from the past into consideration, since it is a time sequence and the future time steps are unknown. 
The normalized attention coefficients are calculated as 

%normalization of attention coefficients
\begin{equation}
\alpha_{ij} = \frac{exp(e_{ij})}{\sum_{k=1}^{T} exp(e_{ik})}
\end{equation}
with the attention coefficients
%attention coefficients
\begin{equation}
e_{ij} = \boldsymbol{v}_a^T tanh(\boldsymbol{W}_a \boldsymbol{s}_{i-1} + \boldsymbol{U}_a \boldsymbol{h}_j).
\end{equation}

The previous hidden state from the decoder $\boldsymbol{s}_{i-1}$ is multiplied by the weight matrix $\boldsymbol{W}_a$ and the the hidden state at time step $j$ from the encoder is multiplied by $\boldsymbol{U}_a$. After applying a $tanh$ function as activation function, the vector $\boldsymbol{v}_a$ scales the term down to a scalar which results in the attention coefficient $e_{ij}$. Note that this attention mechanism is similar to the spatial attention for the GAT layer in section \ref{sec:gat_layer}. 

Now the sequnce is encoded into hidden states and the attention mechanism selects the relevant hidden states from the past time steps. The decoder, which consists also of an GRU, takes the context vector $\boldsymbol{c}_i$ in each time step and calculates, based on the previous hidden state $\boldsymbol{s}_{i-1}$ and the previous output $\boldsymbol{y}_{i-1}$, the new hidden state $\boldsymbol{s}_{i}$ and the current output $\boldsymbol{y}_{i}$. Generally, the decoder has the same structure as the encoder. The new hidden state is calculated as

\begin{equation}
	\boldsymbol{s}_i = (1-\boldsymbol{z}_i) \circ \boldsymbol{s}_{i-1} + \boldsymbol{z}_i \circ \boldsymbol{\tilde{s}}_i
\end{equation}
where the proposal hidden state, the update gate and the reset gate are calculated as
\begin{equation}
	\begin{split}
	\boldsymbol{\tilde{s}}_i =& tanh(\boldsymbol{W}^{\prime} \boldsymbol{y}_{i-1} + \boldsymbol{U}^{\prime} [\boldsymbol{r}_i \circ \boldsymbol{s}_{i-1}] + \boldsymbol{C}^{\prime} \boldsymbol{c}_i + \boldsymbol{b}^{\prime}) \\
	\boldsymbol{z}_i = &\sigma(\boldsymbol{W}_z^{\prime} \boldsymbol{y}_{i-1} + \boldsymbol{U}_z^{\prime} \boldsymbol{s}_{i-1} + \boldsymbol{C}_z^{\prime} \boldsymbol{c}_i + \boldsymbol{b}_z^{\prime}) \\
	\boldsymbol{r}_i = &\sigma(\boldsymbol{W}_r^{\prime} \boldsymbol{y}_{i-1} + \boldsymbol{U}_r^{\prime} \boldsymbol{s}_{i-1} + \boldsymbol{C}_r^{\prime} \boldsymbol{c}_i + \boldsymbol{b}_r^{\prime}).
	\end{split}
\end{equation}

The notation $(\cdot)^{\prime}$ at the weight matrices means, that these are different to the weight matrices for the encoder in section \ref{sec:RNN}. Furthermore, the context vector $\boldsymbol{c}$ is taken into consideration and weighted by the matrices $\boldsymbol{C}^{\prime}$, $\boldsymbol{C}_z^{\prime}$ and $\boldsymbol{C}_r^{\prime}$. The initial input vector $\boldsymbol{y}_0$ is set to a zero-vector. The initial hidden state for the decoder is determined as $\boldsymbol{s}_0 = tanh(\boldsymbol{W}_s^{\prime} \boldsymbol{h}_1)$, where $\boldsymbol{W}_s^{\prime}$ is a trainable weight matrix. Except of this modification the calculation of the new hidden state is similar to the presented GRU in section \ref{sec:RNN}. To calculate the output for the specific time step $i$, the decoder GRU is extended with a single output layer:

\begin{equation}
	\boldsymbol{y}_i = \sigma(\boldsymbol{W}_o^{\prime} \boldsymbol{y}_{i-1} + \boldsymbol{U}_o^{\prime} \boldsymbol{s}_{i-1} + \boldsymbol{C}_o^{\prime} \boldsymbol{c}_i + \boldsymbol{b}_o).
\end{equation}

This layer computes, based on the previous output $\boldsymbol{y}_{i-1}$, hidden state $\boldsymbol{s}_{i-1}$ and current context vector $\boldsymbol{c}$ the current output for time step $i$ which is part of the output sequence \cite{bahdanau_neural_2014}.

In this chapter the basics of feedforward and recurrent neural networks as well as the RNN encoder-decoder algorithm is presented. Based on this methods, it is possible to create an approach for solving the task of queue length estimation in road networks. Also the presented attention mechanisms for spatial correlation (see GAT layer in section \ref{sec:gat_layer}) and temporal correlations in the sequence (this section) help to be potential superior to classic approaches like the method after \cite{liu_real-time_2009} presented in chapter \ref{sec.liu_method}.


\section{Implementation} \label{sec.DL_implementation}

The theoretical background for implementing the deep learning model was presented in  section \ref{sec:basics_NN}. In this section, the focus is on the implementation of these methods to create a deep learning model in the programming language Python. Furthermore, the procedure for generating the dataset, which is used for training, validation and testing, is presented.

There has been a lot of progress in the recent years regarding software tools, which are developed to simplify the implementation of powerful deep learning applications. The most common software library in Python, which is used in the field of deep learning, is \textit{Tensorflow} \cite{martin_abadi_tensorflow:_2015}. It is an open source software library which is developed to perform numerical computation on a wide range of platforms (e.g. CPUs and GPUs on desktop computers but also on server clusters). It was originally developed by the Google Brain Team and became open source in 2015. Another important Python software library in this field is \textit{Keras} \cite{chollet_keras_2015}. The goal of Keras is to provide a high-level API (application program interface), which simplifies the implementation of machine learning and deep learning solutions even more. With Keras it is possible to prototype solutions very fast and generate early results. The focus of Keras is on user friendliness, modularity and easy extensibility by custom layers. Keras works on top of other, more fundamental, deep learning libraries like Tensorflow or Theano. In this thesis, the high-level API Keras is used with Tensorflow as backend. That means, all the code written with Keras is converted to Tensorflow code, which runs then as Python code on the CPU or GPU. 
 
Another important part of the implementation is to create a graph, which is an abstract representation of the road network topology. The knowledge about the graph is crucial for the graph attention layer used in the deep learning model. Fortunately, SUMO is able to export the structure of the road network as a graph using the open source Python library \textit{NetworkX} \cite{hagberg_exploring_2008}. In NetworkX it is possible to have an abstract representation of the road network as a NetworkX-graph which consists of nodes and edges. The nodes are the lanes, since they are the objects of interests with information about traffic. The lanes are connected by intersections, so in this case the intersections are represented by edges. This method of abstraction is visualized in fig. \ref{bild.NetworkX}.

%create figure which is similar to the poster from Matt
\begin{figure}[H]
	\centering
	\includegraphics[width=1\textwidth]{deeplearning/networkX.pdf}
	\caption[Abstracting graph with nodes and edges from rod network] {Abstracting graph with nodes and edges from road network; (a) represents the classic road network in SUMO; (b) visualizes the graph representation with nodes and edges \cite{wright_geometric_2018}. } \label{bild.NetworkX}
\end{figure}

On the right side (a), the classic road network with only one lane for each direction (to keep it simple) is presented. Each lane represents a node with a certain number from 1 to 8. These lanes are connected by the intersection. The figure (b) visualizes the abstracted graph representation for this example intersection. The ellipses represent the nodes (lanes with each number) which are connected by edges (straight lines). For instance cars that arrive on lane 1 in figure (a): They can leave the intersection either on lane 8 (right turn), lane 6 (straight) or lane 4 (left turn). Looking at figure (b), the node 1 is connected by arrows to node 8, 6 and 4. In this particular case it is a \textit{directed graph}, since the edges have a direction (e.g. cars can only change from lane 1 to 8 but not vice versa). If the edges do not have a certain direction, it is called an \textit{undirected graph}. The library NetworkX provides a function to abstract the adjacency matrix from the graph. In case of the example in fig. \ref{bild.NetworkX}, the adjacency matrix would be
\begin{equation}
	A =  \begin{pmatrix} 
	0 & 0 & 0 & 1 & 0 & 1 & 0 & 1 \\
	0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
	0 & 1 & 0 & 0 & 0 & 1 & 0 & 1 \\
	0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
	0 & 1 & 0 & 1 & 0 & 0 & 0 & 1 \\
	0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
	0 & 1 & 0 & 1 & 0 & 1 & 0 & 0 \\
	0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 
	\end{pmatrix}.
\end{equation}

For the usage in the graph attention layer, it is necessary to add the presented adjacency matrix to an identity matrix of the same size, so that the main diagonal of the matrix are ones. Just by that, each lane is able to consider also its own features as input rather than just its neighbors. Of course for larger road networks, like in this thesis, the road networks have more lanes and the adjacency matrix $A$ becomes larger. Especially for this thesis, $A$ includes the upstream and downstream connections of each lane, but not the neighboring lanes which are eligible for lane changing. So this is a good point to start, since the complexity of the adjacency matrix is not too high. The calculated adjacency matrix is then an input for the GAT layer and does not change over time. This is how the spatial structure of the road network is provided to the deep learning model.

The other very important input for the deep learning model are the features. In this particular approach, eight input features for each lane for every time step are used. The first six features come from the e1-detectors in SUMO, which include the \textit{number of contributed vehicles}, \textit{occupancy} and the \textit{speed} of the vehicles for the stop bar and the advanced detector. The e1 detectors provide the data for every second. The seventh input is the information about the traffic light signal at the end of the lane. It is a second-by-second binary signal which is one, if the traffic light is green and zero otherwise. The eighth feature is the estimation results of the method after \cite{liu_real-time_2009} presented in chapter \ref{sec.liu_method}. Although the estimation of this method is not accurate on larger road networks due to lane changing and stop an go traffic, it can help to guide the estimation in the right direction. The information provided by this method is just the maximum queue length for an entire traffic light cycle. Therefore, it is necessary to process a linear interpolation between the maximum length, to create second-by-second data as well.
Once, the second-by-second data for the whole simulation for every lane are collected, the features have to be gathered in a design matrix $\boldsymbol{X}$. The design matrix is assembled to the shape $[simulations \times timesteps \times lanes \times features]$. Generally, this is an array of four dimensions, where the features for each time step are collected for each lane and put together in a two dimensional matrix. In the deep learning field a four dimensional vector is also often called a \textit{tensor}. Furthermore, this is done for every time step of the simulation, which yields the third dimension. Finally, data from multiple simulations can be fed into the network, which results then in the fourth dimension. 
The same procedure can be executed for building the $Y$ array, which has the same structure except of replacing the features with the targets. In this approach the number of targets is two. The first target is the maximum queue length measured by the e2-detector in SUMO. The algorithm gives us the ground-truth data of the maximum queue length for each traffic light cycle. To get second-by-second data, a linear interpolation has to be made between the data points. The second target is the number of vehicles that are on the entire lane, and it is not relevant if they are part of the queue or not. These data can be provided by the e2-detector as well by extracting the value \textit{nVehSeen} for each second. Finally, the structure of $\boldsymbol{Y}$ is $[simulations \times timesteps \times lanes \times targets]$

\begin{figure}[h]
	\centering
	\includegraphics[width=0.6\textwidth]{deeplearning/model_topology.pdf}
	\caption[Topology of the deep learning model] {Topology of the deep learning model. } \label{bild.DL_model}
\end{figure}

After building $\boldsymbol{X}$ and $\boldsymbol{Y}$, the second-by-second data can be averaged over a certain time interval. In this thesis the time interval is chosen to be 10 seconds. By that, the size of the input data is reduced and the information density increased. $\boldsymbol{X}$ and $\boldsymbol{Y}$ can  now be used to train the model. The used model structure is shown in fig. \ref{bild.DL_model}.
The design matrix $\boldsymbol{X}$ is fed into the first GAT layer, which is supposed to learn spatial attention between the lanes. As a second input, the GAT layer receives the adjacency matrix $\boldsymbol{A}$. In fig. \ref{bild.DL_model} only one GAT layer for simplicity is shown. In the final approach two GAT layer are stacked together behind each other. The number of output features for both GAT layer is chosen to be 128, which was determined iteratively by trial and error. Generally, it is recommended to choose the number of features as a power of two to optimize storage usage. Since the GAT layer only take a matrix of the dimension $lanes \times features$ as an input to process the learning algorithm presented in \ref{sec:gat_layer}, wrapper-code is necessary, which feeds in the matrix for all time steps and for all simulations [$\forall simulations, \forall timesteps$]. The following Dense layer are fully connected layer which are presented in sec. \ref{sec:basics_NN}. The dense layer with the width of 128 are supposed to rearrange the learned features from the GAT layer in a way it is necessary for the following encoder-decoder structure. For this layer, the same wrapper-code is necessary, since fully connected layer only take a matrix as input. Following, the encoder takes the whole data for each simulation as an input, including the time steps. So for the encoder, the wrapper code is not necessary anymore, since the encoder handles the time steps sequentially (see sec. \ref{sec:enc-dec}). The inputs per time step are encoded to hidden states, which are used by the following attention decoder to decode the hidden states back into the output time sequence. The temporal attention mechanism is included in the decoder. Both, the encoder and attention decoder, have 128 units per hidden state. Generally, in this approach two different attention mechanism are used. In the GAT layer spatial attention is applied, while the decoder uses temporal attention to estimate the output sequence. 
Furthermore, $L^2$ regularization and dropout (see sec. \ref{sec:basics_NN}) after each GAT and dense layer are applied to avoid overfitting. During training, the loss function for the optimization algorithm is chosen as the mean squared error (MSE) between the prediction and the ground-truth data.

The entire procedure for training and testing the deep learning model starts with running several traffic simulations (e.g. 150) with all the same settings in SUMO and collecting for each of them the detector data. The single SUMO simulations are all different from each other although they have the same settings, since the traffic in SUMO is randomized. The used road network in SUMO is exactly the same then in sec. \ref{sec.liu_on_grid}. Based on the detector data the queue length estimation after chapter \ref{sec.liu_method} is executed for each simulation. Afterwards the collection of simulations are divided into training, validation as well as the test data and the $\boldsymbol{X}$ and $\boldsymbol{Y}$ matrices are build. During training, the gradient updates for the parameter are calculated based on the training data. The validation data are also used during training to calculate the validation loss and monitoring the success of the training regarding under- or overfitting. After the training is finished, the model is tested on the test data, which it has never seen before during training, to evaluate the performance. The results of this test data are presented in the following chapter. 

%-----------------------------------------------------------------------------
%Implementation:
%
%-> talk briefly about keras and tensorflow in python

%-> describe how a road network is modeled as a graph

%-> introduce model topology with arrangement of gat layer -> dense -> enc-dec

%-> describe time distributed wrapper

\section{Results} \label{sec.DL_results}

In this chapter the results of the introduced deep learning model are presented. The first part is about the practical usage of the mean average error (MAPE), and which problems result based on that. Furthermore, an alternative metric for evaluation, the \textit{mean average error} is introduced. Afterwards, the results from selected lanes are presented and the performance of the deep learning model is compared to the method of \cite{liu_real-time_2009}. In addition to that, the overall performance for the entire network for multiple simulations is presented. Afterwards, the difference of the estimation accuracy is discussed, in case the results from the method presented in \ref{sec.liu_method} (here in future called \textit{Liu-method}) is not an input feature for the deep learning model. Finally, the performance of the model is validated in case traffic light cycles or traffic arrival flow changes for the test data, compared to the training data. 

\begin{figure}[h]
	\centering
	\includegraphics[width=1\textwidth]{deeplearning/20181009_0_A_normal_run1_251/DL_result_queue_0-1to0-2_2.pdf}
	\caption[Example for not reliable MAPE] {
		Example for not reliable MAPE: \\
				\begin{tabular}{c|c|c|} 
					\cline{2-3}
					& \multicolumn{2}{c|}{\textbf{Queue estimation:}} \\
					& \textbf{DL model}     & \textbf{Liu-method}     \\ \hline
					\multicolumn{1}{|c|}{MAE {[}m{]}}           & 15                  & 67.1          \\ \hline
					\multicolumn{1}{|c|}{MAPE {[}\%{]}} & 190.9                  & 53.4           \\ \hline
				\end{tabular}
				} \label{bild.MAPE_problem}
\end{figure}

Before the final results are presented, it is important to emphasize the limitations of the MAPE for evaluation of the performance. Due to the fact that the MAPE measures the percentage error, the metric is not reliable anymore, when the ground-truth value goes close to zero, while the estimation has a larger value. This correlation is presented in fig. \ref{bild.MAPE_problem}, which is a real prediction from the trained DL model. The MAPE of the DL model (190.9\%) is worse than the MAPE of the Liu-method (53.4\%), although the DL model has a much better performance considering the impression of the graph in fig. \ref{bild.MAPE_problem}. The reason for that is located at the beginning of the time axis after 200 seconds. The ground-truth value is close to zero, while the estimated value of the DL model is at around 20 meters. Considering the the formula of the MAPE which is

\begin{equation}
MAPE = \frac{1}{m} \sum_{m} \bigm| \frac{Observation - Estimation}{Observation} \bigm| \times 100 \%,
\end{equation}

the phenomenon can be explained. When the observation is close to zero but the estimation is not, the result of the fraction becomes very high and does not represent the real performance of the estimation anymore. An alternative is the \textit{mean average error (MAE)}

\begin{equation}
	MAE = \frac{1}{m} \sum_{m} \bigm| Observation - Estimation \bigm|.
\end{equation}

The MAE does not have the problem of the exploding value in some cases, and is still interpretable, since it has the same dimension as the estimation (in this case meters or number of vehicle). Regarding fig. \ref{bild.MAPE_problem}, the MAE for the DL model is 15.0 meters while for the Liu-method 67.1 meters. In the following both metrics (MAPE and MAE) are presented, but in some cases the MAPE does not give reliable results.
In fig. \ref{bild.compare_simus} the results for another lane in the network are presented. Figure \ref{bild.compare_simus} (a) shows the estimated queue length from the DL model and Liu-method compared to the ground-truth data in the upper graph. The performance of the deep learning model is very accurate, it follows the ground-truth data very well. Especially the two maximums at 500 and 800 seconds are good estimated.
\begin{figure}[H]
	\centering
	\includegraphics[width=1\textwidth]{deeplearning/20181009_0_A_normal_run1_251/2_2to1_2.pdf}
	\caption[Comparison of results for the same lane from different test simulations] {Comparison of results for the same lane from different test simulations (DL model is the same). \\
		\begin{tabular}{c|c|c|c|}
			\cline{2-4}
			& \multicolumn{2}{c|}{\textbf{Queue estimation:}} & \textbf{nVehSeen:} \\
			& \textbf{DL model}     & \textbf{Liu-method}     & \textbf{DL model}  \\ \hline
			\multicolumn{1}{|c|}{MAE (a)}           & 10.5 m                & 43.2 m                  & 1.9 veh            \\ \hline
			\multicolumn{1}{|c|}{MAPE (a) {[}\%{]}} & 24.7                  & 59.3                    & 61124881.6         \\ \hline
			\multicolumn{1}{|c|}{MAE (b)}           & 13.2 m                & 31.8 m                  & 1.3 veh            \\ \hline
			\multicolumn{1}{|c|}{MAPE (b) {[}\%{]}} & 27.2                  & 50.4                    & 50774859.8         \\ \hline
		\end{tabular}} \label{bild.compare_simus}
\end{figure}
This is also represented by the MAPE (24.7\%) and MAE (10.5 m). The Liu-method underestimates, which is caused by the effect of stop-and-go traffic, discussed in sec. \ref{sec.liu_on_grid}, since the presented lane is a left-turn lane. 
The breakpoint C is detected too early, which results in continuous underestimation. The MAPE for the Liu-method is 59.3\% and the MAE 43.2 meter, which attest the better performance of the DL model. The Liu-method has the same issue for almost every left-turn lane in the road-network.
In the lower graph of (a) the estimation for the number of vehicles on the entire lane are shown. Due to the fact, that second-by-second data are used which are averaged to 10 second intervals, the graph seems to have a higher resolution than the upper graph for the queue length, where only one value per traffic light cycle is linear interpolated. Generally, the ground frequency depends on the traffic light phases. The neural network is able to detect the frequency and tries to estimate the peaks, which is not everywhere accurate. With a MAE of 1.9 vehicle (the MAPE is not reliable in this case), the performance is acceptable, but not perfect yet. 
In fig. \ref{bild.compare_simus} (b) results for exact the same lane in the same road network are shown. They are predicted by the same DL model, just for another test simulation. 
\begin{figure}[H]
	\centering
	\includegraphics[width=1\textwidth]{deeplearning/right_turn_example.pdf}
	\caption[Estimation results for a right-turn lane] {Estimation results for a right-turn lane. \\
		\begin{tabular}{c|c|c|c|}
			\cline{2-4}
			& \multicolumn{2}{c|}{\textbf{Queue estimation:}} & \textbf{nVehSeen:} \\
			& \textbf{DL model}     & \textbf{Liu-method}     & \textbf{DL model}  \\ \hline
			\multicolumn{1}{|c|}{MAE}           & 4.8 m                 & 19.8 m                  & 1.9 veh            \\ \hline
			\multicolumn{1}{|c|}{MAPE {[}\%{]}} & 16.5                  & 77.3                    & 33.9               \\ \hline
		\end{tabular}} \label{bild.right_turn_exmpl}
\end{figure}
This should emphasize two things: First, the simulation data generated by SUMO, which are used for training, validation and testing, are very different from each other. The goal is to have a high diversity in the data, so that the deep learning model is able to generalize knowledge and does not overfit.  
Second, although the DL model performs very well in (a), it has still a satisfying performance in (b) for a completely different ground-truth, which is also caused by the high diversity in the training data. The MAPE for the queue length in (b) is 27.2\% and the MAE is 13.2 meters. The Liu-method also suffers here from the stop-and-go traffic and underestimates.
In fig. \ref{bild.right_turn_exmpl} an example for a right-turn lane is shown. In this case, the DL model has satisfying performance with a MAPE of 16.5\% (MAE = 4.8 m), although it starts to "smooth out" after 1000 seconds. This effect could be caused by to many time steps that are taken into consideration for the decoding. The Liu-method is overestimating, since the lane is a right-turn lane where a lot of lane changes occur. Vehicles are changing after passing the advanced detector to other lanes, which cannot be handled by the Liu-method (discussed in sec. \ref{sec.liu_on_grid}). This is also shown by the MAPE (77.3\%) and MAE (19.8 m). For the estimation of nVehSeen, the curve is again smoothing and not very accurate. The MAPE (33.9\%) and MAE (1.9 veh) is also not completely satisfying. Also this could be caused by to many time steps, that are taken into consideration for the attention decoding. Especially for estimating the second target (nVehSeen), the optimal model configuration is not found yet. However, note that the approach has a lot of potential so far. This is also emphasized by considering the averaged MAPE and MAE for the entire road network (not only for a single lane, as presented above). In table \ref{tab.MAE_entire_net} the MAEs for several test simulations are presented. The MAPEs are not reliable sources, since at least one lane has a MAPE which has a very high (and not reliable) value.

\begin{table}[h]
	\centering
	\begin{tabular}{c|c|c|c}
		& \multicolumn{2}{c|}{\textbf{MAE queue length {[}m{]}}} & \textbf{MAE nVehSeen {[}veh{]}} \\ \hline
		\textbf{Simulation \#} & \textbf{DL model}         & \textbf{Liu-method}        & \textbf{DL model}               \\ \hline
		1                      & 9.1                       & 18.1                       & 1.4                             \\
		2                      & 9.5                       & 17.8                       & 1.5                             \\
		3                      & 9.0                       & 18.6                       & 1.6                             \\
		4                      & 8.9                       & 18.1                       & 1.4                             \\
		5                      & 9.4                       & 18.5                       & 1.5                             \\ \hline
		\textbf{Average:}      & 9.2                       & 18.2                       & 1.5                            
	\end{tabular}
	\caption[Estimation results (MAE) of an entire road-network] {Estimation results (MAE) of an entire road-network for five test simulations.} \label{tab.MAE_entire_net}
\end{table}

It turns out, that the performance of the deep learning model is very constant over different independent test simulations. In addition to that, the DL model has around twice better performance regarding the MAE than the Liu-method. For the number of vehicles on the entire lane (nVehSeen), the deep learning model has a MAPE around 1.5 vehicles, which is acceptable considering the number of vehicles that are on the entire lane, but there is no reference to other methods available.  

\subsection{Robustness for different Arrival Rates}

Although the performance, especially of the queue length estimation, is satisfying, it is important to note that the traffic parameter are the same for training and testing. For example the arrival rate of the traffic is the same, although the traffic routes for the single vehicles are randomized by SUMO. It would be interesting to analyze, how the DL model behaves when the input data have different arrival rates. This study is shown in fig. \ref{bild.03_period} for a selected left-turn lane.

\begin{figure}[h]
	\centering
	\includegraphics[width=1\textwidth]{deeplearning/03_period_test.pdf}
	\caption[Test of the DL model for different traffic arrival rate] {Test of the DL model for different traffic arrival rate.\\
\begin{tabular}{c|c|c|c|}
	\cline{2-4}
	& \multicolumn{2}{c|}{\textbf{Queue estimation:}} & \textbf{nVehSeen:} \\
	& \textbf{DL model}     & \textbf{Liu-method}     & \textbf{DL model}  \\ \hline
	\multicolumn{1}{|c|}{MAE}           & 75.6 m                & 149.6 m                 & 13.9 veh           \\ \hline
	\multicolumn{1}{|c|}{MAPE {[}\%{]}} & 45.6                  & 63.7                    & 148.5              \\ \hline
\end{tabular}
} \label{bild.03_period}
\end{figure}

The presented test data have a arrival rate of 3.33 veh/s while the DL model is only trained on data with 2.5 veh/s arrival rate. Regarding the estimation of the queue length, the DL model has some problems to estimate accurately the first maximum. But it still has with a MAE of 75.6 meters a better performance than the Liu-method with MAE = 149.6. The estimation of the nVehSeen is more critical. In the period of time between 650 and 1150 seconds, the estimated vehicles on the lane reach very high values. The DL model shows instable behavior. However, this behavior is expected, since it has never seen a nVehSeen of 20 during training before. So it has no knowledge about how to handle this situation. This is a common problem for any sort of statistical model which is used for prediction out of samples. The worse performance is also illustrated by the average MAEs for all lanes. The MAE for the DL model is 31.5 m, for the Liu-method 56.2 m and for the DL model estimating the nVehSeen the MAE is 5.9. 

\begin{figure}[H]
	\centering
	\includegraphics[width=1\textwidth]{deeplearning/03_period_test_new.pdf}
	\caption[Test of the DL model for traffic arrival rate of 0.3 sec/veh, when model is trained on multiple arrival rates] {Test of the DL model for traffic arrival rate of 0.3 sec/veh, when model is trained on multiple arrival rates.\\
		\begin{tabular}{c|c|c|c|}
			\cline{2-4}
			& \multicolumn{2}{c|}{\textbf{Queue estimation:}} & \textbf{nVehSeen:} \\
			& \textbf{DL model}     & \textbf{Liu-method}     & \textbf{DL model}  \\ \hline
			\multicolumn{1}{|c|}{MAE}           & 77.8 m                & 149.5 m                 & 4.4 veh           \\ \hline
			\multicolumn{1}{|c|}{MAPE {[}\%{]}} & 39.4                 & 63.7                    & 61.3              \\ \hline
		\end{tabular}\label{bild.03_period_new}
	} 
\end{figure}

The performance can be improved, if the model is not only trained with simulation data based on a specific arrival rate, but with a high diversity of arrival rates. If the deep learning model has a higher diversity in the training data, the generalization of knowledge is better. In fig. \ref{bild.03_period_new} the results are shown for the same DL model but trained with 180 simulations with a randomized arrival rate between 0.45 and 0.25 sec/veh for each simulation, rather than with 125 simulations of 0.4 sec/veh data as for fig. \ref{bild.03_period}. Since the data have a higher diversity, more simulations are necessary to allow similar performance. 

The performance of the queue length estimation in fig. \ref{bild.03_period_new} is not better compared to fig. \ref{bild.03_period} which has a MAE of (75.6 m). The reason is that 180 simulations are too less for training a model properly for all possible arrival rates. But it is still enough to stabilize the prediction for nVehSeen in the lower graph of fig. \ref{bild.03_period_new}. While in fig. \ref{bild.03_period} the nVehSeen becomes unstable and have a MAE of 13.9 veh, in fig. \ref{bild.03_period_new} the behavior is stable with a MAE of 4.4 veh. The model has already seen similar traffic situations during training and can handle the situation. The average MAEs for the entire network are compared in table \ref{tab.compare} for both different models.

\begin{table}[H] 
	\centering
	\begin{tabular}{|c|c|c|c|c|}
		\hline
		\multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Arrival rate\\  for training\\ {[}sec/veh{]}\end{tabular}}} & \multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Number of\\ training \\ simulations\end{tabular}}} & \multicolumn{2}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Queue estimation\\ MAE\\ (MAD)\end{tabular}}}                   & \textbf{\begin{tabular}[c]{@{}c@{}}nVehSeen\\ MAE\\ (MAD)\end{tabular}} \\ \cline{3-5} 
		&                                                                                                       & \textbf{DL model}                                          & \textbf{Liu-method}                                       & \textbf{DL model}                                                       \\ \hline
		\textbf{0.4}                                                                                                   & \textbf{125}                                                                                          & \begin{tabular}[c]{@{}c@{}}31.5 m \\ (30.2 m)\end{tabular} & \begin{tabular}[c]{@{}c@{}}56.2 m\\ (66.4 m)\end{tabular} & \begin{tabular}[c]{@{}c@{}}5.9 veh\\ (6.8 veh)\end{tabular}             \\ \hline
		\textbf{0.25 - 0.45}                                                                                           & \textbf{180}                                                                                          & \begin{tabular}[c]{@{}c@{}}24.7 m\\ (21.1 m)\end{tabular}  & \begin{tabular}[c]{@{}c@{}}56.2 m\\ (66.4 m)\end{tabular} & \begin{tabular}[c]{@{}c@{}}3.8 veh\\ (3.2 veh)\end{tabular}             \\ \hline
	\end{tabular}
	\caption[MAEs and MADs for the entire road network predicted by the same model which was trained on datasets with different arrival rates] {MAEs and MADs for the entire road network predicted by the same model which was trained on datasets with different arrival rates.} \label{tab.compare}
\end{table}

The MAE for the queue estimation is better for the deep learning model trained on multiple arrival rates compared to the model trained on only one arrival rate. Even better is the improvement for the estimated nVehSeen. As additional metric the \textit{mean absolute deviation (MAD)} is used, which is 
\begin{equation}
	MAD = \frac{1}{m} \sum_{i = 1}^{m} \mid MAE_i - \overline{MAE} \mid,
\end{equation}
where $m$ is the number of lanes and $\overline{MAE}$ is the average MAE for all lanes. The MAD is very high for both models due to the instable situations that occur for both. Still, the model trained on more arrival rates, has a lower MAD in all categories. 
 Furthermore, the DL model does not become instable in certain situations anymore. While for the old model on 16 of 120 lanes instability occurs, the improved model has 5 lanes where the nVehSeen becomes instable and overestimation occurs. The improved model has not the optimal performance yet, since a higher amount of simulations are necessary to gain reliability.
However, this demonstration should emphasize how important it is to train on many different relevant data as possible to have a maximum of generalized knowledge for every traffic case.

% show how dl model performs on changed traffic light cycles(optional if time left)
%train DL model with different traffic light cycles (optinal)

%-> verify that using the results from liu are gaining the accuracy of the estimation -> come to the conclusion, that it was worth it to do the preliminary work with liu

\subsection{Influence of Liu-Method as Input}

Finally, it is also important to investigate, if the usage of the Liu-method as an input feature is a benefit. Therefore, the exactly same model was trained twice. For the first dataset the results of the Liu-method were included (8 input features) which is in the following called \textit{with-Liu model}, for the second dataset the Liu-method was not included (7 input features) also called as \textit{no-Liu model}. 
In fig. \ref{bild.without_liu} the results of both training sessions are presented for the same lane. In fig. \ref{bild.without_liu} (a) the estimated queue length and nVehSeen for the model with Liu-method as input are presented, while in (b) the results for the model without Liu-method are shown. For the comparison of the estimated queue length, the no-Liu model with a MAE of 32.9 m seems to have almost the same performance as the with-Liu model with a MAE of 31.1 m. 
\begin{figure}[H]
	\centering
	\includegraphics[width=1\textwidth]{deeplearning/compare_w_wo_liu/figure_comparison.pdf}
	\caption[Comparison of results for the same lane if results of Liu-method are input feature or not] {Comparison of results for the same lane if results of Liu-method are input feature or not (DL model is the same). \\
		\begin{tabular}{c|c|c|c|}
			\cline{2-4}
			& \multicolumn{2}{c|}{\textbf{Queue estimation:}} & \textbf{nVehSeen:} \\
			& \textbf{DL model}     & \textbf{Liu-method}     & \textbf{DL model}  \\ \hline
			\multicolumn{1}{|c|}{MAE (a)}           & 31.1 m                & 121.7 m                  & 2.0 veh            \\ \hline
			\multicolumn{1}{|c|}{MAPE (a) {[}\%{]}} & 18.86                  & 68.2                    & 64.6         \\ \hline
			\multicolumn{1}{|c|}{MAE (b)}           & 32.9 m                & 121.8 m                  & 2.3 veh            \\ \hline
			\multicolumn{1}{|c|}{MAPE (b) {[}\%{]}} & 21.5                  & 68.2                    & 40.9         \\ \hline
		\end{tabular}} \label{bild.without_liu}
\end{figure}

The comparison between the estimated nVehSeen is more interesting: While the MAEs are also not significant different (2.0 veh for with-Liu and 2.3 veh for no-Liu) the difference between the graphs are higher. The nVehSeen in (a) (with-Liu) follow the ground truth curve quiet well with a slightly smoothing character. For the nVehSeen in (b) (no-Liu), the behavior of the estimation becomes sometimes instable with many drops, at some points the estimation is even below zero. It is suspected, that this unrealistic behavior is caused by overfitting of the training data. Not only on this particular lane, but also on 15 other lanes the estimated value drops 25 times in total below zero. This does not happen for the DL model in trained with the Liu-method as input. The average MAEs as well as the MADs of both models are compared in table \ref{tab.MAE_wo_liu}. 

\begin{table}[h]
	\centering
	\begin{tabular}{|c|c|c|c|c|}
		\hline
		\multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Usage\\ of\\ Liu-method\end{tabular}}} & \multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Number of\\ training \\ simulations\end{tabular}}} & \multicolumn{2}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Queue estimation\\ MAE\\ (MAD)\end{tabular}}}                 & \textbf{\begin{tabular}[c]{@{}c@{}}nVehSeen\\ MAE\\ (MAD)\end{tabular}} \\ \cline{3-5} 
		&                                                                                                       & \textbf{DL model}                                        & \textbf{Liu-method}                                       & \textbf{DL model}                                                       \\ \hline
		\textbf{w/ Liu}                                                                           & \textbf{125}                                                                                          & \begin{tabular}[c]{@{}c@{}}9.4 m \\ (5.3 m)\end{tabular} & \begin{tabular}[c]{@{}c@{}}18.1 m\\ (13.7 m)\end{tabular} & \begin{tabular}[c]{@{}c@{}}1.6 veh\\ (0.4 veh)\end{tabular}             \\ \hline
		\textbf{w/o Liu}                                                                          & \textbf{125}                                                                                          & \begin{tabular}[c]{@{}c@{}}9.0 m\\ (5.4 m)\end{tabular}  & \begin{tabular}[c]{@{}c@{}}18.1 m\\ (13.7 m)\end{tabular} & \begin{tabular}[c]{@{}c@{}}1.4 veh\\ (0.4 veh)\end{tabular}             \\ \hline
	\end{tabular}
	\caption[Estimation results (MAE) for model with and without Liu-method as input] {Estimation results (MAE) for model with and without Liu-method as input.} \label{tab.MAE_wo_liu}
\end{table}

Only considering the MAEs, the no-Liu model seems to be slightly better. Furthermore, there is no difference for the MADs between both models. However, this data do not represent the performance regarding the stability for the estimation of nVehSeen. The Liu-method used as input feature prevents the model from overfitting, which results in a more stable behavior of nVehSeen. In this case, prior knowledge about the traffic is used, to avoid overfitting and guide the model in the right direction. In this case, to add prior knowledge has similar effects than classic regularization techniques like dropout or $L^2$-Regularization. It would be also possible to avoid overfitting by using more training data, but in reality traffic data are rare and expensive. So it is beneficial for the learning process to have preprocessed data by the Liu-method as input, which saves some effort for data mining and computational cost for training. 

% --------------write stuff-----------------
%Results: (similar structure to presentation)
%
%-> present problem with MAPE and introduce MAE
%
%-> show results for different simulations for the same lane
%
%-> Present average MAPE and MAE for the entire road network
%
%-> try to improve performance by implementing attention horizon in attention decoder (not so important)
%
%-> test the model with different traffic light plans
%
%-> verify that using the results from liu are gaining the accuracy of the estimation -> come to the conclusion, that it was worth it to do the preliminary work with liu





==> implementation/implementation.tex <==
\chapter{Implementation and Results}
hk
\section{Implementation of Conventional Estimation}
fhd
\section{Implementation of Deep Learning Estimator}
gjk
